Distributed Algorithms from Arboreal Ants for the Shortest Path Problem

Colonies of the arboreal turtle ant create networks of trails that link nests and food sources on the graph formed by branches and vines in the canopy of the tropical forest. Ants put down a volatile pheromone on edges as they traverse them. At each vertex, the next edge to traverse is chosen using a decision rule based on the current pheromone level. There is a bidirectional flow of ants around the network. In a field study, Chandrasekhar et al. (2021) observed that the trail networks approximately minimize the number of vertices, thus solving a variant of the popular shortest path problem without any central control and with minimal computational resources. We propose a biologically plausible model, based on a variant of the reinforced random walk on a graph, which explains this observation and suggests surprising algorithms for the shortest path problem and its variants. Through simulations and analysis, we show that when the rate of flow of ants does not change, the dynamics converges to the path with the minimum number of vertices, as observed in the field. The dynamics converges to the shortest path when the rate of flow increases with time, so the colony can solve the shortest path problem merely by increasing the flow rate. We also show that to guarantee convergence to the shortest path, bidirectional flow and a decision rule dividing the flow in proportion to the pheromone level are necessary, but convergence to approximately short paths is possible with other decision rules.

==> Old_stuff/old_intro.tex <==

\section{Introduction}

%general intro on ants
Collective behavior is widespread in nature. Global behavior operates without central control using simple local interactions among individuals. Well known examples include the coordinated movement of schools of fish and flocks of birds \autocite{couzin2005effective}.  Such behavior is based on biological distributed algorithms \autocite{navlakha2011algorithms} that have raised questions of interest in theoretical computer science, for example opinion dynamics and bird flocking \autocite{chazelle2009natural,chazelle2012dynamics,bhattacharyya2013convergence}.

A recent focus of research on collective behavior is how it is tuned to changing environmental conditions \autocite{gordon2016evolution}. Social insects such as ants live in colonies that function collectively. The 14K species of ants  that live in very diverse habitats provide an opportunity to learn how local conditions have shaped the evolution of the algorithms that regulate collective behavior.  


Here we examine how local interactions generate trail networks in arboreal ants. Many ant species create networks of foraging trails. The arboreal turtle ant {\em C. goniodontus} nests and forages in trees, its trail networks constrained to lie on a natural graph formed by tangled branches and vines in the tree canopy.
Turtle ants form a routing backbone of foraging trails linking several nests and temporary food sources.  The backbone trail network can be large, extending hundreds of meters, spanning many trees and using many junctions in dense vegetation. The colony chooses paths from amongst a wide range of possibilities, constrained by the graph structure of the vegetation. Ants lay trail pheromone as they move along the edges, and this pheromone guides their choice of edges to traverse.

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-10pt}
  \begin{center}
\includegraphics[width=0.5\textwidth]{ants_pic.jpg}
  \end{center}
\vspace{-8pt}
\captionof{figure}{\small{Tangled branches in which the turtle ants forage. Picture from \textcite{chandrasekhar2018distributed}.}}
%\label{fig:ants2_graph}
\vspace{-13pt}
\end{wrapfigure}

\textcite{chandrasekhar2018distributed} proposed a biologically feasible distributed algorithm that could plausibly describe how these ants with limited memory maintain the routing backbone and find alternative paths to circumvent broken links in the backbone, communicating only through pheromone without a specific targeted recipient.
They model the movement of each ant as a Markov process on an undirected graph which must choose an edge to traverse at each vertex (junction) based on the pheromone levels detected.
The traversal of an edge by an ant reinforces the pheromone level of that edge (additively); this pheromone also decays with time (multiplicatively).
%They were interested in whether such an algorithm finds short paths and converges to a single consensus path.
They identified local decision rules for selecting edges to traverse which (in simulations) resulted in trail networks with short paths with low entropy (a measure of convergence towards a single consensus path).


More recently, \textcite{chandrasekhar2019better} used data from field observations of the trail networks of turtle ants to test what objective functions these trails may be optimizing. 
%to edit
They identified each vertex or junction in the vegetation where an ant had a choice among more than one edge in the direction it was traveling. They measured the length of each edge. They also measured variation among vertices in physical configuration by assigning  a transition index to each transition from one edge through a vertex to another edge, to indicate the likelihood of successive ants taking the same trajectory through the vertex and thus reinforcing it with pheromone.
%To evaluate how the ants choose nodes and edges from the options provided by the surrounding vegetation, they also mapped all nodes, measured all edges, and assigned transition indices, for all possible paths up to five nodes away from each node used by the ants.

Their conclusion was that the ants’ networks favored the maintenance of coherent trails over choosing shortest paths. In particular, the ants' trails  were more likely to maximize the probability of rapid reinforcement with pheromone , and  minimize the number of vertices, than minimizing the distance travelled.
They reasoned that maximizing the probability of reinforcement and minimizing the number of vertices contribute to coherence because they both diminish the risk of losing ants from the trail.
Trail networks must balance exploration (necessary for the colony to construct trails, search for new resources, repair breaks) and coherence. 
%to edit
There is a small probability of exploration at each vertex; thus, minimizing the number of vertices traversed reduces opportunities for the ants to get lost.
They also point out that the algorithm proposed in their previous work \autocite{chandrasekhar2018distributed} did not distinguish between minimizing the number of vertices and the distance traveled, and that further work is needed to develop an algorithm that captures the role of physical variation in the configuration of the vertices in the environment.

Here we address  this by developing a simple model for how ants form a trail that explicitly accounts for exploration at vertices of the network that results in the loss of ants. Our model builds on \textcite{chandrasekhar2018distributed}.  
%Technically, we use flows to model the rate of arrival of ants instead of individual ants.
We model trails as a bidirectional flow from nest to food source and back, and model ants getting lost by leakage.
Our flows are akin to flows in traffic networks for example \autocite{wardrop1952road, beckmann1955studies, roughgarden2002bad}.
We start with the linear decision rule, where the flow divides among the next set of edges in proportion to their pheromone level.
Starting from the original graph, we show that the dynamics under this linear decision rule converges to the path with minimum leakage.
Previous studies  have also shown that Argentine  ants sometimes find shortest paths \autocite{goss1989self}. We show that in our model, the same dynamics converges to the shortest path if the flow is increasing with time.
Note that the rate of flow of ants is positively reinforced by the detection of food sources and other factors \autocite{deneubourg1986random,gordon2012dynamics};
we show that such increasing flow actually leads to convergence to the shortest path. This suggests that, at least in principle, ants have the ability to obtain information about path length by varying their flow rate. It would be fascinating to explore experimentally whether ants actually use this ability to find the shortest path. We prove these results for a network consisting of two parallel paths, a case that has received some attention in the literature \autocite{goss1989self, dorigo2001experimental}.
Our simulations indicate that the dynamics converge for general graphs drawn from various random graph models.

The bidirectional nature of flow is crucial for our results. 
This is different from the traditional theoretical computer science literature where the flows considered  are usually unidirectional.
In the case of unidirectional flow, we show that no pheromone based rule can find the shortest or minimum leakage path.
However bidirectional flow is characteristic of many biological networks, including ant trails, %slime molds?,  
and is also found in engineered systems such as telecommunication networks. 
%[Can you find an example from routing networks?] 
For example, bidirectional flow in the ant trail network was essential for the ability to repair breaks in \textcite{chandrasekhar2018distributed}.

Our convergence results are for the linear decision rule. To understand the dynamics for non-linear rules, we consider a very general family of decision rules. We show that the linear decision rule is the unique member of this family with guaranteed convergence properties to the minimum leakage and shortest paths.
%To understand the dynamics for non-linear rules, we identify the stable equilibrium states for a very general family of decision rules. We show that change in flow is necessary for any rule in this family to be able to converge to the shortest path. We also show that the linear decision rule is the unique member of this family with guaranteed convergence properties to the minimum leakage and shortest paths.

%For this family of rules

The model we study has some resemblance to reinforced random walks introduced by Diaconis and others, that have received some attention in the literature \autocite{diaconis1980finetti,davis1990reinforced,pemantle2007survey},
%Reinforced random walks (both edge- and vertex-reinforced variants) 
and have found applications in biology
\autocite{stevens1997aggregation,coding2008random,smouse2010stochastic}.
Here a single agent traverses a graph by choosing edges with probability proportional to their edge weight (analogous to pheromone). This edge weight increases additively each time the edge is traversed. However, there are a few key differences between the model we study and the setup for reinforced random walks:
1) We have a large number of ants in the system (modeled by a flow) and their behavior is affected by their collective actions ,while the model for reinforced random-walks considers a single agent whose behavior is influenced by its past random choices.
2) Pheromone decays geometrically over time in our model, but edge weights do not decrease in reinforced-random walks. 
3) Our model has leakage at each vertex, and this is not present in the setup for reinforced-random walks.

Nevertheless, the model we propose and study is a Markov process of particular relevance to biology, in a similar spirit to random walk like processes studied before. Despite the apparent simplicity of our model, analyzing its behavior is surprisingly non-trivial. 
Our goal is to introduce this process and make a first attempt at understanding its properties. The behavior of this process in simulations suggests that it should be possible to significantly generalize the results we prove here.
We think our work raises fascinating questions that we hope will be interesting to both computer scientists and biologists.


==> Old_stuff/old_results.tex <==
\begin{comment}
We describe our results in this section. In Section \ref{sec:parallel_paths_ub}, we consider the dynamics for the linear decision rule. Through simulations and analysis, we show that when the incoming forward and backward flows do not change with time, the flow dynamics converge to the path with the minimum leakage. When the incoming forward and backward flows are increasing,  in the absence of leakage, the dynamics converge to the shortest path. This demonstrates that, at least in principle, ants have the ability to obtain information about path length by changing their flow rate.

These results raise several questions.  How important is the bi-directional nature of flow? How would the dynamics behave when we use some non-linear decision rule? We try to understand these questions in \Cref{sec:general_rules_lb}.

First, we show that the bi-directional flow is indeed necessary for convergence to the shortest path or the minimum leakage path for any pheromone based decision rule. We then consider a very general family of decision rules. We show that one cannot guarantee convergence to the shortest or the minimum leakage path for any non-linear decision rule in this family. That is, the linear decision rule is the only member of this family with \emph{guaranteed convergence} to the shortest or the minimum leakage path. 

Does it mean that the usefulness of the forces of increasing flow and leakage is only restricted to the linear decision rule? Through simulation with various non-linear decision rules, we observe that for most graph instances, the path found in the presence of these forces has length (respectively leakage) smaller than or equal to the length (respectively leakage) of the path found in their absence. This suggests that the usefulness of increasing flow and leakage in finding desirable paths is not limited to the linear decision rule.
%We then identify the stable equilibrium states for a very general family of rules. Building on this understanding of the equilibrium states, we argue that there is no advantage of using non-linear decision rules if the goal is to find the shortest path or the path with minimum leakage.
\end{comment}

==> equilibriumstates.tex <==
\textbf{Equilibrium for general rules. }
Here we try to understand more general decision rules beyond the linear rule discussed in the last subsection. To do this, we first identify the equilibrium states and their stability for a very general class of decision rules,  when there is no leakage and the forward and backward flow levels are fixed. We do this for the case of two parallel paths from $s$ to $d$. These rules essentially distributed the forward (backward) flow among the outgoing (incoming) edges of any vertex, based on the normalized pheromone levels at these edges. We assume that these rules are continuous in the sense that a small change in the pheromone level will not lead to a large change in the proportions of the flow distributed. We also assume that these rules are monotone in the sense that increasing the normalized pheromone level at any edge will never decrease the proportion of flow entering that edge. As both these properties seem reasonable, the class of rules considered is sufficiently general.

\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
\includegraphics[width=0.35\textwidth]{ants2-crop.pdf}
  \end{center}
\vspace{-8pt}
\captionof{figure}{\small{Equilibria for general rules.}}
\label{fig:ants2_graph}
\vspace{-10pt}
\end{wrapfigure}

More formally, we consider the family of rules given by functions $g:[0,1/2] \rightarrow [0,1] \in \setflb$. For any vertex with out-degree (in-degree) $1$, these rules send the forward (backward) flow to the next (previous) vertex, just as in the case of linear rules. For any vertex with out-degree (in-degree) $2$,   these rules use the function $g:[0,1/2] \rightarrow [0,1]$, which takes the minimum of the  normalized pheromone levels on the two outgoing (incoming)  edges, and returns the fraction of the forward (backward) flow on the edge with minimum pheromone level. We assume that  $g$ is monotonically increasing, that is, $g(x) \leq g(x')$ for all  $x \leq x'$. Further, $g$ satisfies $g(0)=0$ and $g(1/2)=1/2$. The last condition basically says that if one of the edges has $0$ normalized pheromone, we do not send any flow on it, and if both the edges have equal pheromone level, then we send equal flow on them.
%we consider are the set of all symmetric, continuous, monotone, normalized pheromone level based rules on the 2 parallel path graph. Formally, any rule $g \in \setflb$ satisfies the following:
\begin{comment}
\begin{itemize}
    \item The rule $g$ is symmetric, that is, the same rule apply to both $s$ and $d$.
    \item The rule $g:[0,1/2] \rightarrow [0,1]$ is pheromone ratio based, meaning at all time steps it takes the minimum of the two normalized pheromone levels on edges belonging to the two paths and returns the fraction of the flow on the minimum edge.
    \item The rule $g$ is monotonically non-decreasing, meaning $g(x) \leq g(x')$ for all $x,x' \in [0,1/2]$ and $x \leq x'$. Further, $g$ satisfies $g(0)=0$ and $g(1/2)=1/2$.
\end{itemize}
\end{comment}
%\shivam{Also mention that there is only one linear decision rule in this family, $g(x) = x$.}


%\shivam{Write a line or two about why this class is interesting. I will do it later.}
Note that the linear decision rule studied in previous subsection belongs to $\setflb$, and corresponds to $g(x) = x$. Next, we understand the equilibrium states under these rules. We start by providing some definitions. 


In the setting of the fixed flow we provide the following definitions\footnote{Note for the case of changing flow it is slightly tricky to define the equilibrium case and requires introduction of normalized flows and pheromones levels. For the purposes of stating our results and to reduce the complexity of the reading we just define the equilibrium state for the fixed flow setting.}. The \emph{state} of the system at time $t$ is the tuple $(\pt,\ft,\bt)$, where $\pt,\ft,\bt \in \R_{\geq 0}^{E}$ are the vectors denoting the pheromone levels, forward and backward flow on the edges E respectively. We say the system has reached an \emph{equilibrium state} at time $t$, if for all $t' \geq t$ the state of the system at time $t'$ is same as $t$. Further an equilibrium state $(\pftt,\ftt,\btt)$ is \emph{stable} if there exists an $\epsilon >0$, such that the system with all initial state $(\pfz,\fz,\bz)$ satisfying\footnote{The condition $(\pftt-\epsilon,\ftt-\epsilon,\btt-\epsilon) \leq (\pfz,\fz,\bz) \leq (\pftt+\epsilon,\ftt+\epsilon,\btt+\epsilon)$ denotes $\pfz_{uv} \in (\pftt_{uv}-\epsilon,\pftt_{uv}+\epsilon)$, $\fz_{uv} \in (\ftt_{uv}-\epsilon,\ftt_{uv}+\epsilon)$, $\bz_{uv} \in (\btt_{uv}-\epsilon,\btt_{uv}+\epsilon)$ for all $(u,v) \in E$.} $(\pftt-\epsilon,\ftt-\epsilon,\btt-\epsilon) \leq (\pfz,\fz,\bz) \leq (\pftt+\epsilon,\ftt+\epsilon,\btt+\epsilon)$ converges to the equilibrium state $(\pftt,\ftt,\btt)$. For the graph with two paths, as the in and out degree of all the edges except $(s,s_1),(s,s_2),(d,d_1),(d,d_2)$ (see \Cref{fig:path_graph}) is exactly one, the dynamics governed by the decision rule $g \in \setflb$ is independent of the pheromone level on these edges. Therefore the state of the two path case is sufficiently represented by the forward and backward flow on all the edges and just the pheromone levels on edges $(s,s_1),(s,s_2),(d,d_1),(d,d_2)$.


Now consider any $g \in \setflb$, let $F_{g}\defeq \{x \in [0,1/2]~|~g(x)=x\}$ be the set of all fixed points. Also let $S_{g}\defeq \{r \in F_{g}~|~\text{there exists }\epsilon>0 \text{ s.t}, ~g(s)<s \text{ for all } s\leq r+\epsilon \text{ and }g(s)>s \text{ for all } s\geq r-\epsilon\}$ \footnote{Note that, $0 \in S_{g}$ if $~g(s)<s$  for all $s\leq r+\epsilon$. Similarly, $1/2 \in S_{g}$ if $~g(s)>s$  for all $s\geq r-\epsilon$}. In the following result we identify the equilibrium states of the dynamics under the decision rule $g$ under the setting of fixed flow and no leakage.
\begin{theorem}\label{thm:grule}
Consider the graph $G$ consisting of two parallel paths $P_1$ and $P_2$ from $s$ to $d$. In the setting of fixed flow and no leakage, the flow dynamics on $G$ governed by the decision rule $g \in \setflb$ has the following properties. For every $r \in F_{g}$, the state of the system is an equilibrium state if the pheromone and flow values are such that: 
    \begin{itemize}
        \item The pheromone levels on all the edges of the top path are equal to $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot r$ and bottom path are equal to $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d}) \cdot (1-r)$.
        \item The forward flows on the top and bottom path are $\fflow{s}\cdot r$ and $\fflow{s}\cdot (1-r)$ respectively.
        \item The backward flows on the top and bottom path are $\bflow{d}\cdot r$ and $\bflow{d}\cdot (1-r)$ respectively.
    \end{itemize}
     Further if $r \in S_{g}$, then such a state of the system is also a stable equilibrium state.
\end{theorem}
\begin{comment}
\begin{figure}[h]
\centering
\includegraphics[scale=0.3]{ants2-crop.pdf}
\caption{Characterization of general rules.}
\label{fig:ants2_graph}
\end{figure}
\end{comment}
See \Cref{fig:ants2_graph} for a pictorial representation of the equilibrium points.




































\subsection{Proof for the stable equilibrium for general rules (\Cref{thm:grule})}
For convenience, we recall some definitions already stated in \Cref{sec:general_rules_lb}. Let $\setflb$ be the set of all symmetric, continuous, monotone, pheromone ratio based rules on the 2 parallel path graph; formally any $g \in \setflb$ satisfy the following:
\begin{itemize}
    \item The rule $g$ is symmetric, that is, the same rule apply to both $s$ and $d$.
    \item The rule $g:[0,1/2] \rightarrow [0,1]$ is pheromone ratio based, meaning at all time steps it takes the minimum of the two normalized pheromone levels on edges belonging to the two paths and returns the fraction of the flow on the minimum edge.
    \item The rule $g$ is monotonically non-decreasing, meaning $g(x) \leq g(x')$ for all $x,x' \in [0,1/2]$ and $x \leq x'$. Further, $g$ satisfies $g(0)=0$ and $g(1/2)=1/2$.
\end{itemize}

For any $g \in \setflb$, let $F_{g}\defeq \{x \in [0,1/2]~|~g(x)=x \}$ and $S_{g}\defeq \{r \in F_{g}~|~\text{there exists }\epsilon>0 \text{ that satisfies}, ~g(s)<s \text{ for all } s\leq r+\epsilon \text{ and }g(s)>s \text{ for all } s\geq r-\epsilon\}$. For $r \in S_{g}$, we use $r_{\epsilon}>0$ to denote a number that satisfies the conditions of the set $S_{g}$, that is,   
$g(s)<s \text{ for all } s\leq r+r_\epsilon \text{ and }g(s)>s \text{ for all } s\geq r-r_\epsilon$. 


\begin{lemma}\label{lem:stable}
Consider the graph $G$ consisting of two parallel paths $P_1$ and $P_2$ from $s$ to $d$. In the setting of fixed flow and no leakage, the flow dynamics on $G$ governed by the decision rule $g \in \setflb$ satisfies the following. For every $r\in S_{g}$ and $\epsp \leq r_{\epsilon}$ if the configuration at time $t \geq 0$ satisfies,
\begin{itemize}
    \item $\npsso(t),\npddo(t)\in (r-\epsp,r+\epsp)$ and $\fflow{uv}(t) \in \fflow{s} \cdot (r-\epsp,r+\epsp)$, $\bflow{uv}(t) \in \bflow{d} \cdot (r-\epsp,r+\epsp)$  for all $(u,v) \in P_{1}$,
    \item $\npsst(t),\npddt(t)\in (1-r-\epsp,1-r+\epsp)$ and $\fflow{uv}(t) \in \fflow{s} \cdot (1-r-\epsp,1-r+\epsp)$, $\bflow{uv}(t) \in \bflow{d} \cdot (1-r-\epsp,1-r+\epsp)$  for all $(u,v) \in P_{2}$~.
\end{itemize}
then at $t+1$ it satisfies,
\begin{itemize}
    \item $\npsso(t+1),\npddo(t+1)\in (r-\epsp,r+\epsp)$ and $\fflow{uv}(t+1) \in \fflow{s} \cdot (r-\epsp,r+\epsp)$, $\bflow{uv}(t+1) \in \bflow{d} \cdot (r-\epsp,r+\epsp)$  for all $(u,v) \in P_{1}$,
    \item $\npsst(t+1),\npddt(t+1)\in (1-r-\epsp,1-r+\epsp)$ and $\fflow{uv}(t+1) \in \fflow{s} \cdot (1-r-\epsp,1-r+\epsp)$, $\bflow{uv}(t+1) \in \bflow{d} \cdot (1-r-\epsp,1-r+\epsp)$  for all $(u,v) \in P_{2}$~.
\end{itemize}
Further if $\epsp \geq \epspp>0$, then the following stronger guarantees hold,
\begin{align*}
    &\npsso(t+1),\npddo(t+1)\in (r-\epsp+c_{g,r,\epspp}\cdot B,r+\epsp-c_{g,r,\epspp}\cdot B),\\  
    &\npsst(t+1),\npddt(t+1)\in (1-r-\epsp+c_{g,r,\epspp}\cdot B,1-r+\epsp-c_{g,r,\epspp}\cdot B),
\end{align*}
where $c_{g,r,\epspp}\defeq \min_{\epspp \leq x \leq r_{\epsilon}} \min(g(r-x)-(r-x),(r+x)-g(r+x))$ and $B$ are fixed constants independent of $\epsp$ and $t$.
\end{lemma}
\begin{proof}
For $r\in S_{g}$, let $\epsp \leq r_{\epsilon}$. We first show that $r-\epsp \leq \npsso(t+1) \leq r+\epsp$. Recall the definition of $\npsso(t+1)$,
\begin{align}
\npsso(t+1)=\frac{\psso(t+1)}{\psso(t+1)+\psst(t+1)} &= \frac{ \psso(t) + 
    \fsso(t) +  \fsos(t)}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)}
\end{align}
We know by the conditions of the lemma that,
\begin{equation}\label{eq:one}
r-\epsp \leq \frac{\psso(t)}{\psst(t)+\psso(t)} \leq r+\epsp~. 
\end{equation}
Also note that,
\begin{equation}\label{eq:two}
r-\epsp \leq \frac{  
    \fsos(t)}{ \fsts(t)+\fsos(t)} \leq r+\epsp~.    
\end{equation}
In the above inequality we used the monotonically non-decreasing property of $x/(1+x)$ and the conditions provided by the induction step at time $t$, that is $\fsos(t)\in \bflow{d} \cdot (r-\epsp,r+\epsp)$ and $\fsts(t)\in \bflow{d} \cdot (1-r-\epsp,1-r+\epsp)$. 

\newcommand{\cle}{c_{g,r}}
\newcommand{\cue}{c_{g,r}}

Using \Cref{eq:one,eq:two} it is immediate that,
$$r-\epsp \leq \npsso(t+1) \leq r+\epsp~.$$
As $\npsso(t+1)+\npsst(t+1)=1$, the above inequalities further imply,
$$1-r-\epsp \leq \npsst(t+1) \leq 1-r+\epsp~.$$
Similar analysis also holds for edges $(d,d_1)$ and $(d,d_2)$. As $\epsp \leq r_\epsilon$, from the definition of $g$ we also have that,
$$\fsso(t+1) \in \fflow{s}\cdot (r-\epsp,r+\epsp)~,$$
which implies $\fflow{uv}(t) \in \fflow{s} \cdot (r-\epsp,r+\epsp)$ for all $(u,v) \in P_{1}$. From the flow conservation property, we immediately get that, $\fflow{uv}(t) \in \fflow{s} \cdot (1-r-\epsp,1-r+\epsp)$ for all $(u,v) \in P_{2}$.
Similar proof holds for the edges $(d,d_1), (d,d_{2})$ and the backward flow;

Recall the definition of $c_{g,r}$ and note that the following bounds hold on the flow values,
\begin{equation}
    \fsso(t) = \fflow{s} \cdot g(\npsso(t)) \leq  \fflow{s}\cdot g(r+\epsp) \leq \fflow{s}\cdot(r+\epsp-\cue)~,
\end{equation}
\begin{equation}
    \fsso(t) = \fflow{s} \cdot g(\npsso(t)) \geq \fflow{s} \cdot g(r-\epsp) \geq \fflow{s}\cdot (r-\epsp+\cle)~.
\end{equation}
Using these bounds, we provide an upper bound for the normalized pheromone level.
\begin{align}
\npsso(t+1)&= \frac{ \psso(t) + 
    \fsso(t) +  \fsos(t)}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)},\\
    & \leq (r+\epsp)+\frac{\fsso(t)-(r+\epsp)(\fsso(t) +  \fsst(t))}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)},\\
    & \leq (r+\epsp)+\frac{\fsso(t)-(r+\epsp)\cdot \fflow{s}}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)},\\
    & \leq (r+\epsp)+\frac{
    \fflow{s}\left( r+\epsp-\cue-r-\epsp\right)}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)},\\
    & \leq (r+\epsp)-\frac{\cue
    \fflow{s}}{ \psst(t) + \psso(t)+ \fsst(t) +\fsso(t) +  \fsts(t)+\fsos(t)},\\
    &\leq (r+\epsp)-\cue\cdot B_1~.
\end{align}
where $B_1\geq 0$ is a fixed constant independent of time $t$ and $\epsp$. Note that in the final expression we used the fact that all the terms in the denominator can be upper bounded by functions of $\fflow{s}, \bflow{d},\delta$ and pheromone levels at time $0$.

Similar analysis as above also gives us,
$$\npsso(t+1)\geq r-\epsp+\cue\cdot B_2~,$$
where $B_2$ is again a fixed constant independent of time $t$ and $\epsp$. Choose $B'=\min(B_1,B_2)$ then we get,
$$\npsso(t+1) \in (r-\epsp+ \cue\cdot B',r+\epsp-\cue\cdot B')~,$$
equivalently we also have,
$$\npsst(t+1) \in (1-r-\epsp+\cue\cdot B',1-r+\epsp-\cue\cdot B')~,$$
Similar analysis also holds for edges $(d,d_1),(d,d_2)$ and we get that,
$$\npddo(t+1) \in (r-\epsp+ \cue\cdot B'',r+\epsp-\cue\cdot B'')~,\quad \npddt(t+1) \in (1-r-\epsp+\cue\cdot B'',1-r+\epsp-\cue\cdot B'')~,$$
where $B''$ is a constant independent of time $t$ and $\epsp$. Further choosing $B=min(B',B'')$, we get the result stated in the lemma. We conclude the proof.
\end{proof}

\renewcommand{\epsp}{\epsilon}

We are now ready to prove the main theorem of this section.

\begin{proof}[Proof of \Cref{thm:grule}]
The proof for the first property is pretty straightforward. Consider any $r \in F_{g}$, we want to show that the state of the system provided in the lemma is an equilibrium state and we do it by induction. 

\paragraph{Hypothesis:}The pheromone and flow values at time $t\geq 0$ satisfy the following: 
    \begin{itemize}
        \item The pheromone levels on all the edges of the top path are equal to $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot r$ and bottom path are equal to $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d}) \cdot (1-r)$.
        \item The forward flows on the top and bottom path are $\fflow{s}\cdot r$ and $\fflow{s}\cdot (1-r)$ respectively.
        \item The backward flows on the top and bottom path are $\bflow{d}\cdot r$ and $\bflow{d}\cdot (1-r)$ respectively.
    \end{itemize}

\paragraph{Base case:} The hypothesis holds for time $t=0$ because of the condition provided by the lemma.

\paragraph{Induction step:} Here we prove the hypothesis for time $t+1$.
Consider any edge $(u,v)$ on the top path, then
\begin{align}
    p_{uv}(t+1)&=\delta \left(p_{uv}(t)+\fflow{uv}(t)+\bflow{uv}(t) \right)~,\\
    &=\delta \left(\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot r+ \fflow{s}\cdot r + \bflow{d} \cdot r\right)~,\\
    &=\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot r~.\\
\end{align}
As the normalized pheromone level on edges $(s,s_{1})$ and $(d,d_{1})$ is $r$, we have that $\fflow{s}\cdot r$ and $\bflow{d}\cdot r$ enters to the top path from the left and right side respectively. Equivalently, $\fflow{s}\cdot (1-r)$ and $\bflow{d}\cdot (1-r)$ enters to the bottom path from the left and right side respectively; by induction we conclude the proof for the first property.

In the remainder we prove the second property about stable equilibrium.  Consider any $\epsilon''>0$, let $r_{\epsilon}>0$ to denote a number that satisfies the conditions of the set $S_{g}$, that is,   
$g(s)<s \text{ for all } s\leq r+r_\epsilon \text{ and }g(s)>s \text{ for all } s\geq r-r_\epsilon$. Denote the equilibrium state mentioned in the lemma by the tuple $(p,f,b)$, where $p$ is the vector of pheromone levels and $f,b$ are the vector of forward and backward flows. In the remainder, we show that $(p,f,b)$ is a stable equilibrium. Choose $\epsilon=r_{\epsilon}$, we show that any initial state $(p(0),f(0),b(0))$ satisfying $(\pftt-\epsilon,\ftt-\epsilon,\btt-\epsilon) \leq (\pfz,\fz,\bz) \leq (\pftt+\epsilon,\ftt+\epsilon,\btt+\epsilon)$ converges to the equilibrium state $(\pftt,\ftt,\btt)$. 

\renewcommand{\epspp}{\epsilon''}
\renewcommand{\epsp}{\epsilon'}
Consider any $\epsilon'' \geq 0$, we show that there exists a time $t_{\epspp}$ such that for all $t \geq t_{\epspp}$, we have that $(\pftt-\epspp,\ftt-\epspp,\btt-\epspp) \leq (p(t),\ft,\bt) \leq (\pftt+\epspp,\ftt+\epspp,\btt+\epspp)$.

Note that the normalized pheromone level and the flows on the edges satisfy the conditions of the \Cref{lem:stable} for parameter $\epsp=\epsilon$. Further, by the guarantees provided by the lemma the normalized pheromone level and the flows on the edges keep satisfying the conditions of the \Cref{lem:stable} for all the future time steps with parameter $\epsp=\epsilon$. Further by the stronger conditions guaranteed by the lemma, we have that the normalized pheromone levels on the edges $(s,s_1), (d,d_1)$ lie in the range $(r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$ for all the future time steps, where $c_{g,r,x}\defeq \min_{\epspp \leq x \leq r_{\epsilon}} \min(g(r-x)-(r-x),(r+x)-g(r+x))$ and $B$ are fixed constants independent of $\epsp$ and $t$. As the normalized pheromone levels lie in the range $(r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$, $r \in S_{g}$ and $\epsilon-c_{g,r,1/2\epspp} \leq \epsilon \leq r_{\epsilon}$, we have that the flow entering into the top path from the left and right sides lie in the range $\fflow{s}\cdot (r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$ and $\bflow{d}(r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$
respectively for all the future time steps. After $max(n,m)$ time steps we have that the normalized pheromone levels lie in the range $(r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$. As $r \in S_{g}$ and $\epsilon-c_{g,r,1/2\epspp} \leq \epsilon \leq r_{\epsilon}$, we have that the flow entering into the top path from the left and right sides lie in the range $\fflow{s}\cdot (r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$ and $\bflow{d}(r-\epsilon+c_{g,r,1/2\epspp}\cdot B,r+\epsilon-c_{g,r,1/2\epspp}\cdot B)$
respectively. Therefore after $\max(m,n)$ times we have made progress and reduce the size of the interval for the normalized and the flow values. Applying the same analysis repeatedly for $O(\frac{\epsilon-1/2\epspp}{c_{g,r,1/2\epspp}\cdot B})$, we get that for all the future time steps the normalized pheromone levels on the edges $(s,s_1),(d,d_1)$ lie in the range $(r-1/2\epspp,r+1/2\epspp)$. The forward flows on the top and bottom path lie in the range $\fflow{s}\cdot (r-1/2\epspp,r+1/2\epspp)$ and $\fflow{s}\cdot (1-r-1/2\epspp,1-r+1/2\epspp)$ respectively. The backward flows on the top and bottom path lie in the range $\bflow{d}\cdot (r-1/2\epspp,r+1/2\epspp)$ and $\bflow{d}\cdot (1-r-1/2\epspp,1-r+1/2\epspp)$ respectively. The conditions on the flow values ensures that the pheromone level on all the top and bottom edges converge in the range $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot (r-\epspp,r+\epspp)$ and $\frac{\delta}{1-\delta} \cdot (\fflow{s}+\bflow{d})\cdot (1-r-\epspp,1-r+\epspp)$. 

Therefore for every $\epspp>0$, we showed that there exists a time $t_{\epspp}$ such that for all $t \geq t_{\epspp}$, we have that $(\pftt-\epspp,\ftt-\epspp,\btt-\epspp) \leq (p(t),\ft,\bt) \leq (\pftt+\epspp,\ftt+\epspp,\btt+\epspp)$. Therefore the point $(p,f,b)$ is a stable equilibrium and we conclude the proof.

\end{proof} 


==> old_stuff.tex <==
\begin{comment}
We introduce a model for ant trail formation, building upon previous work on biologically feasible local algorithms that plausibly describe how ants maintain trail networks. The model is a variant of a reinforced random walk on a directed graph, where ants lay pheromone on edges as they traverse them and the next edge to traverse is chosen based on the level of pheromone; this pheromone decays with time. There is a bidirectional flow of ants in the network: the forward flow proceeds along forward edges from source (e.g. the nest) to sink (e.g. a food source), and the backward flow in the opposite direction. Some fraction of ants are lost as they pass through each vertex (modeling the loss of ants due to exploration observed in the field). We initiate a theoretical study of this model. We note that ant navigation has inspired the field of ant colony optimization, heuristics that have been applied to several combinatorial optimization problems; however the algorithms developed there are considerably more complex and not constrained to being biologically feasible.

We first consider the linear decision rule, where the flow divides itself among the next set of edges in proportion to their pheromone level. Here, we show that the process converges to the path with minimum leakage when the forward and backward flows do not change over time. On the other hand, when the forward and backward flows increase over time (caused by positive reinforcement from the discovery of a food source, for example), we show that the process converges to the shortest path. These results are for graphs consisting of two parallel paths (a case that has been investigated before in experiments). Through simulations, we show that these results hold for more general graphs drawn from various random graph models; proving this convergence in the general case is an interesting open problem.  Further, to understand the behaviour of other decision rules beyond the linear rule, we consider a general family of decision rules. For this family, we show that there is no advantage of using a non-linear decision rule, if the goal is to find the shortest or the minimum leakage path. We also show that bidirectional flow is necessary for convergence to such paths. Our results provide a plausible explanation for field observations, and open up new avenues for further theoretical and experimental investigation.
\end{comment}


%Despite the simplicity of our model and similarity to other random walk processes studied in the literature, the dynamics of this process are remarkably complex. 
\begin{comment}
Despite the simplicity of our model and similarity to other random walk processes studied in the literature, the dynamics of this simple process are remarkably complex. For a graph consisting of two parallel paths (that has been investigated before in experiments), we study the process where ants choose the next edge with probability proportional to pheromone level. We call such a decision rule the linear decision rule. Here, we show that the process converges to the path with minimum leakage when the rate of the forward and backward flows do not change over time.
On the other hand, when the forward and backward flows increase over time (caused by positive reinforcement from the discovery of a food source, for example), we show that the process converges to the shortest path. Further, to understand the behaviour of other decision rules beyond the linear rule, we identify the equilibrium states for a general family of decision rules. For this family, we show that if the goal is to find the shortest or the minimum leakage path, then there is no advantage of using non-linear decision rule. We also show that bidirectional flow is necessary for convergence to the shortest path or the path with minimum leakage. We report on experiments that show the convergence of this process on more general graphs drawn from various random graph models; proving this convergence in the general case is an interesting open problem.
\end{comment}


\begin{comment}
\section{Related Work}
\paragraph{Ant trails.} 

Our model builds on the work of \textcite{chandrasekhar2018distributed}. They propose a biologically feasible distributed algorithm that could plausibly describe how arboreal turtle ants maintain trail networks, finding alternative paths to circumvent broken links. They also investigate various local decision rules that ants may use for selecting edges to traverse. Among the decision rules considered, they found that the linear decision rule is the most likely to explain the choices ants made in field observations. However, they notice that with the linear decision rule, the dynamics fail to converge to a single consensus path, contradicting field observations where ants regularly converge to a single path. However, we show that under the forces of increasing flow or leakage (which were not considered in \autocite{chandrasekhar2018distributed}), with the linear decision rule, the dynamics always converge to a path. Therefore, our results suggest plausible ways in which these ants can use the linear decision rule and still converge to a path.

There exists a large body of work on understanding trail networks in ant species that forage on 2d surfaces \autocite{watmough1995modelling, helbing1997active, boissard2013trail, fontelos2015pde, amorim2015modeling}. This includes species of army ants  \autocite{deneubourg1989blind}, Argentine ants \autocite{garnier2009path, latty2011structure, flanagan2013fast}, Pharaoh’s ants \autocite{malivckova2015stochastic},  among many others. Unlike arboreal ants, the movement of these ants is not constrained to any graph like structure. However, the fundamental principles behind how the forces of leakage and increasing flow operate are quite general, and might be applicable to some of these species.

Our work is different from traditional ant-colony optimization \autocite{dorigo1991distributed, dorigo2005ant, lopez2018ant}, where the algorithms considered are not required to be biologically plausible. Models of ant colony optimization (ACO) are inspired by ant behavior to solve combinatorial optimization problems, such as the traveling salesman problem and the shortest path problem . In ACO, individual agents (simulating ants) construct candidate solutions using heuristics, and then use limited communication (simulating pheromone) to lead other agents towards better solutions. 
 %Recent advances improve ACO through techniques such as local search, cunning ants, and iterated ants. 
 In ACO, the simulated ants have significantly more computational power than is biologically plausible for real ants. Unlike real ants, the simulated ants have the ability to remember, retrace and reinforce entire paths, and can determine the amount of ``pheromone'' laid by the quality of the global solution. 

\paragraph{Distributed Computing.}
Problems with locality constraints have traditionally been investigated in computer science in the context of distributed systems \autocite{lynch1996distributed}. 
This includes the study of popular graph problems such as the shortest path problem \autocite{chandy1982distributed, elkin2017distributed, ghaffari2018improved, becker2016near}, the minimum spanning tree problem \autocite{pandurangan2018distributed} and various NP-hard problems \autocite{suomela2013survey}. Here, machines, each with a local view of the network, communicate with their neighbors to cooperatively perform a computation. This is different from the locality constraints faced by ants where they only communicate through pheromone. 


\paragraph{Slime mold.} 
 In a surprising experiment, \textcite{nakagaki2000maze} demonstrated that slime mold finds the the shortest path in a maze. In an attempt to understand this phenomenon, \textcite{tero2007mathematical} gave a mathematical model for the dynamics of slime mold. In the slime mold dynamics, current flows from the source vertex to the destination vertex in an electrical resistor network. The diameter of resistors increase in proportion to the current level along them. Here, the diameter of resistors is analogous to the pheromone level at edges in our model. However, beyond this similarity, we are not aware of any other technical connections between the two models.
 
 A series of papers  \autocite{miyaji2007mathematical,miyaji2008physarum, bonifaci2012physarum}  proved convergence to the shortest path for the slime mold dynamics, and various generalizations and surprising connections to other problems have been investigated since then \autocite{straszak2016irls, straszak2016natural, bonifaci2020physarum}. In a similar spirit, our work is an attempt to model train formation in arboreal turtle ants, giving rise to intriguing observations and conjectures, that can potentially lead to an interesting line of research.
\end{comment}

%connections between the  \autocite{miyaji2007mathematical,miyaji2008physarum} began the analytical study of the dynamics showing convergence for a restricted family of graphs. Finally,  \autocite{bonifaci2012physarum} proved that the slime mold dynamics converge to the shortest path for general graphs.   extended this result to show that the slime mold dynamics can be used to solve the  uncapacitated mincost flow problem as well. \autocite{straszak2016irls} showed a connection between the slime mold dynamics and the Iteratively Reweighted Least Squares (IRLS) algorithm used in compressed sensing.  
%Very recently, \autocite{bonifaci2020physarum} introduced and studied a slime model dynamics for the network design problem.
%Slime mold dynamics  have some similarity with the ant dynamics. In the slime mold dynamics, current flows from $s$ to $t$ in a resistor network. The diameter of the resistor increases in proportion to the current level along the resistor. 
 %{ ] showed} that eventually all the current flows through the shortest path.
%Our work can be considered as an effort towards giving a biologically plausible model for ants, with analytical results on some family of graphs, and simulation results for general graphs. It is similar to the work of \autocite{bonifaci2012physarum} on slime molds effect of diameter, and of pheromone level, but there is no obvious similarity in the dynamics.

%Connections to distributed systems. TODO.

    


%\paragraph{Organization:} In \Cref{sec:model}, we provide the mathematical definition of our model for ant trail formation. In \Cref{sec:results}, we state all the main results of our paper. In \Cref{sec:proof_overview}, we provide proof overviews for all our main results and defer the formal proofs to Appendix. %Finally in \Cref{sec:open_problems}, we provide further discussion about the problem and interesting open directions.

\iffalse
Some high level points:
\begin{itemize}
    \item Deborah's recent paper \autocite{chandrasekhar2019better} showed that turtle ants prefer paths with minimum number of vertices. Intuition given in that paper was that more vertices in a path would lead to higher chances of getting lost.
    \item How do ants find such paths with no central control and minimal computational resources? 
    \item Ants use pheromone to communicate.
    \item We model this as bidirectional flow from nest to food source and back, and model ants getting lost by leakage.
    \item Starting from the original graph, we show that the flow converges to the path with minimum leakage.
    \item Previous works have also shown that argentine  ants sometimes find shortest paths \autocite{goss1989self}. We show that in our model, the flow converges to the shortest path if the flow is increasing with time.
    \item We also show fundamental limits for a very general class of pheromone based rules. For example, we show that change in flow is necessary for any continuous monotone pheromone based rule to be able to converge to the shortest path.
    \item The bidirectional nature of flow is crucial for our results. This is different from the traditional TCS literature where the flows considered  are usually unidirectional.
    \item Connections to reinforced-random walks.
    \item Connections to distributed systems.
    \item In the past, \autocite{nakagaki2000maze} experimentally showed that slime mold converges to the shortest paths in a maze. Later, \autocite{tero2007mathematical} gave a mathematical model for slime mold dynamics and showed using simulations that it converges to the shortest path. \autocite{miyaji2007mathematical,miyaji2008physarum} began the analytical study of the dynamics showing convergence for a restricted family of graphs. Finally,  \autocite{bonifaci2012physarum} proved that the slime mold dynamics converge to the shortest path for general graphs.  \autocite{straszak2016natural} extended this result to show that the slime mold dynamics can be used to solve the  uncapacitated mincost flow problem as well. \autocite{straszak2016irls} showed a connection between the slime mold dynamics and the Iteratively Reweighted Least Squares (IRLS) algorithm used in compressed sensing.  
    
    In a similar spirit, our work can be considered as an effort towards giving a biologically plausible model for ants, with analytical results on some family of graphs, and simulation results for general graphs.  Slime mold dynamics also have some similarity with the ant dynamics. In the slime mold dynamics, current flows from s to t in a resistor network. The diameter of the resistor increases in proportion to the current level along the resistor. And they show that eventually all the current flows through the shortest path. Their notion of diameter, and our notion of pheromone level seems similar, but there is no obvious similarity in the dynamics.
    
    \item Our work different from traditional ant-colony optimization, where the algorithms considered are not required to be biologically plausible. From one of Deborah's paper \autocite{chandrasekhar2018distributed}: ``Models of ant colony optimization (ACO), frst proposed in 1991, loosely mimic ant behavior to solve combinatorial optimization problems, such as the traveling salesman problem and the shortest path problem. In ACO, individual ants each use a heuristic to construct candidate solutions, and then use pheromone to lead other ants towards higher quality solutions. Recent advances improve ACO through techniques such as local search, cunning ants, and iterated ants. ACO, however, provides simulated ants more computational power than turtle actually ants possess; in particular, ACO-simulated ants have sufcient memory to remember, retrace, and reinforce entire paths or solutions, and they can choose how much pheromone to lay in retrospect, based on the optimality of the solution''
\end{itemize}
\fi


\begin{comment}
{\sc Earlier Version}
Shortest path problems are amongst the most basic optimization problems on graphs studied in computer science \autocite{ford1956network, bellman1958routing, dijkstra1959note}.
Textbook algorithms for this problem find optimum solutions using knowledge of the entire network \autocite{kleinberg2006algorithm, dasgupta2008algorithms, cormen2009introduction}. In the distributed setting, multiple machines, each with a local view of the network must communicate with their neighbors to cooperatively solve an optimization problem such as shortest path \autocite{lynch1996distributed}.
Biological systems, such as ant trail networks, are fascinating natural examples of such distributed algorithms,
often finding globally optimum solutions using simple local interactions among individuals, devoid of central control. 

Despite their apparent simplicity, understanding why such natural distributed algorithms work is a challenge. Well known examples include  shortest path recovery by slime molds \autocite{nakagaki2000maze, tero2007mathematical, miyaji2007mathematical,miyaji2008physarum, bonifaci2012physarum}, and the coordinated movement of schools of fish and flocks of birds \autocite{couzin2005effective}.  Such collective behavior based on biological distributed algorithms \autocite{navlakha2011algorithms} has raised many questions of interest in computer science \autocite{chazelle2009natural,chazelle2012dynamics, musco2016ant, bhattacharyya2013convergence, straszak2016irls, straszak2016natural, bonifaci2020physarum}.

Here we investigate collective behaviour in arboreal ants and its connections to the shortest path problem. The arboreal turtle ant {\em C. goniodontus} nests and forages in trees, its trail networks constrained to lie on a natural graph formed by tangled branches and vines. In a striking field study, \autocite{chandrasekhar2019better} observed that these ants find paths that approximately minimize the number of vertices between their nest and the food source, essentially solving a variant of the shortest path problem. This potentially reduces their chances of getting lost. 

How ants achieve this is a mystery and this is the motivating question for our work. We develop a model
that gives a plausible answer to this question, and sheds light on many other intriguing phenomena. This
includes a surprising connection between the rate of flow of ants and the length of the path found. We
also demonstrate the crucial role played by bidirectional flow of ants (from nest to food source and back)
in finding such paths. 
The insights from our model may also apply to other domains involving local interactions such as swarm computing and molecular robots \autocite{lund2010molecular, brambilla2013swarm, werfel2014designing, hecker2015beyond}.
\end{comment}
\begin{comment}
{\sc earlier version}

We humans started the formal study of computation in the last century. On the other hand, nature---through evolution---has been ``designing'' algorithms for more than 3.5 billion years. The fascinating aspect of these algorithms is that they often find global solutions using simple local interactions among individuals, without any central control. Well known examples include  shortest path recovery by slime molds \autocite{nakagaki2000maze, tero2007mathematical, miyaji2007mathematical,miyaji2008physarum, bonifaci2012physarum}, and the coordinated movement of schools of fish and flocks of birds \autocite{couzin2005effective}.  Such collective behavior based on biological distributed algorithms \autocite{navlakha2011algorithms} has raised many questions of interest in computer science \autocite{chazelle2009natural,chazelle2012dynamics, musco2016ant, bhattacharyya2013convergence, straszak2016irls, straszak2016natural, bonifaci2020physarum}.

Here we investigate collective behaviour in arboreal ants and its connections to the popular shortest path problem \autocite{ford1956network, bellman1958routing, dijkstra1959note}. 
The arboreal turtle ant {\em C. goniodontus} nests and forages in trees, its trail networks constrained to lie on a natural graph formed by tangled branches and vines. 
In a striking field study, \autocite{chandrasekhar2019better} observed that these ants find paths that approximately minimize the number of vertices between their nest and the food source, potentially reducing the opportunities to get lost. So they  essentially solve a variant of the shortest path problem. 

This raises the following natural question: How do ants find paths which minimize the number of vertices without any central control and with minimal computational resources?
We develop a model that gives a plausible answer to this question, and sheds light on many other intriguing phenomena. This includes a surprising connection between the rate of flow of ants and the length of the path found. We also demonstrate the crucial role played by bidirectional flow of ants (from nest to food source and back) in finding such paths. The insights from our model may also apply to other domains involving local interactions such as swarm computing and molecular robots \autocite{lund2010molecular, brambilla2013swarm, werfel2014designing, hecker2015beyond}.

\end{comment}
\begin{comment}
\dg{Finding the shortest path in a dynamic environment. Here we describe how ants solve this problem with distributed algorithms and no global information. 





Turtle ants create a trail network in a network of vegetation, using pheromone. The arboreal turtle ant {\em C. goniodontus} nests and forages in trees, its trail networks constrained to lie on a natural graph formed by tangled branches and vines in the tree canopy. Ants lay trail pheromone as they move along the edges, and this pheromone guides their choice of edges to traverse. Their trail networks link several nests and temporary food sources, extending hundreds of meters, and spanning many trees in the dense vegetation.The ants travel both ways around a circuit. We consider how changes in the rate of flow of the ants and bidirectional flow contribute to the solution of the shortest path problem.

We start with the linear decision rule, where the flow divides among the next set of edges in proportion to their pheromone level. We consider the setting where incoming forward and backward flow levels do not change with time. In this case, through simulations and analysis, we show that the dynamics converges to the path with minimum leakage. We do these simulations on general graphs drawn from various random graph families, and mathematically analyse the dynamics for  graphs consisting of two parallel paths, a case that has received some attention in the literature \autocite{goss1989self, dorigo2001experimental}. When all the vertices have equal leakage, the path with minimum leakage corresponds to the path with the minimum number of vertices. This result suggests a plausible way in which turtle ants find paths which minimize their probability of getting lost. }


A recent focus of research on collective behavior is how it is tuned to changing environmental conditions \autocite{gordon2016evolution}. Social insects such as ants live in colonies that function collectively. The 14K species of ants  that live in very diverse habitats provide an opportunity to learn how local conditions have shaped the evolution of the algorithms that regulate collective behavior. 
\end{comment}


\begin{comment}

Here we examine how local interactions generate trail networks in arboreal ants. The arboreal turtle ant {\em C. goniodontus} nests and forages in trees, its trail networks constrained to lie on a natural graph formed by tangled branches and vines in the tree canopy. Ants lay trail pheromone as they move along the edges, and this pheromone guides their choice of edges to traverse. Their trail networks link several nests and temporary food sources, extending hundreds of meters, and spanning many trees in the dense vegetation. 


Recently, \textcite{chandrasekhar2019better} used data from field observations of the trail networks to test what objective functions these trails may be optimizing.  They observed that these ants favour paths that minimize the number of vertices, than minimizing the distance travelled. Further, they prefer vertices with physical configuration most likely to be reinforced with pheromone. There is a small probability of exploration at each vertex. Thus, they reasoned that minimizing the number of vertices traversed reduces opportunities for the ants to get lost.  These observations raise the following natural question: \emph{How do turtle ants minimize the number of vertices in their path, without any central control and with minimal computational resources?} 


We develop a model for ant trail formation that gives a plausible answer to this question, and also sheds light on some surprising phenomena. Note that this question is a variant of the popular shortest path problem for which many algorithms exist \autocite{ford1956network, bellman1958routing, dijkstra1959note}, and are regularly taught in undergraduate algorithms classes. In the context of arboreal turtle ants, what makes this question intriguing is that they find such paths without any central control, under the locality constraints posed by nature. The insights from our model may also be applicable to other systems involving locality constraints such as swarm computing and molecular robots \autocite{lund2010molecular, brambilla2013swarm, werfel2014designing, hecker2015beyond}.
\end{comment}

%This is another example of simple local interactions resulting in a global solution, and can have implications for 
 %other domains involving local interactions such as swarm computing and molecular robots.

%\paragraph{Role of increasing flow.}
%In the previous result, we assume that the incoming forward and backward flow levels remain unchanged. \emph{What happens when incoming flows change with time?} 
  

%\paragraph{Importance of bidirectional flow.}
%Our model has bidirectional flow of ants from nest to food source and back. \emph{How crucial is this bidirectional nature of flow?} 
%We do these simulations on general graphs drawn from various random graph families, and mathematically analyse the dynamics for  graphs consisting of two parallel paths, a case that has received some attention in the literature \autocite{goss1989self, dorigo2001experimental}.

%This is different from the traditional computer science literature where the flows considered  are usually unidirectional. %However, bidirectional flow is characteristic of many biological networks, including ant trails, 
%and is also found in engineered systems such as telecommunication networks. 
%For example, bidirectional flow in the ant trail network was essential for the ability to repair breaks in \textcite{chandrasekhar2018distributed}.


%We show that the contribution of increasing flow and leakage to finding the shortest path is not limited to the linear decision rule.

%We think our work opens up fascinating avenues for further theoretical and experimental investigation that will be interesting to both computer scientists and biologists.
%\paragraph{The case of non-linear decision rules.}
%Our convergence results are for the linear decision rule. \emph{How applicable are these convergence results to non-linear rules?} To understand this question, we consider a very general family of decision rules. We show that the linear decision rule is the unique member of this family with guaranteed convergence properties to the minimum leakage and the shortest path. We can view increasing flow and leakage  as two possibly conflicting forces, the former drives the dynamics towards shorter paths while the latter prefers paths with small leakage. Non-linearity in the decision rule can be thought of as another force, possibly in conflict with the forces of leakage and increasing flow, preferring certain states depending on initial pheromone level at the edges. 


%\emph{Does it mean that the usefulness of the forces of increasing flow and leakage is only restricted to the linear decision rule?} Through simulation with various non-linear decision rules, we observe that for most graph instances, the path found in the presence of these forces has length (respectively leakage) smaller than or equal to the length (respectively leakage) of the path found in their absence. This suggests that these forces can be effective even with non-linear decision rules.

\begin{comment}
The model we study has some resemblance to reinforced random walks introduced by Diaconis and others, that have received some attention in the literature \autocite{diaconis1980finetti,davis1990reinforced,pemantle2007survey},
%Reinforced random walks (both edge- and vertex-reinforced variants) 
and have found applications in biology
\autocite{stevens1997aggregation,coding2008random,smouse2010stochastic}.
Here a single agent traverses a graph by choosing edges with probability proportional to their edge weight (analogous to pheromone). This edge weight increases additively each time the edge is traversed. However, there are a few key differences between the model we study and the setup for reinforced random walks:
1) We have a large number of ants in the system (modeled by a flow) and their behavior is affected by their collective actions ,while the model for reinforced random-walks considers a single agent whose behavior is influenced by its past random choices.
2) Pheromone decays geometrically over time in our model, but edge weights do not decrease in reinforced-random walks. 
3) Our model has leakage at each vertex, and this is not present in the setup for reinforced-random walks.

Nevertheless, the model we propose and study is a Markov process of particular relevance to biology, in a similar spirit to random walk like processes studied before. Despite the apparent simplicity of our model, mathematically analyzing its behavior is surprisingly non-trivial. 
Our goal is to introduce this process and make a first attempt at understanding its properties. The behavior of this process in simulations suggests that it should be possible to significantly generalize the results we prove here.
We think our work raises fascinating questions that we hope will be interesting to both computer scientists and biologists.
\end{comment}
%Ants essentially solve a variant of the classic shortest path problem

%
%Our goal is to introduce this process and make a first attempt at understanding its properties. The behavior of this process in simulations suggests that it should be possible to significantly generalize the results we prove here. In particular, we conjecture that our provable convergence results hold for general graphs.

%Our provable convergence results hold only for graphs consisting for parallel paths. We show these convergence results through simulations on many family of graphs. However, we show provable convergence only in the case of parallel paths. We conjecture that provable convergence holds for general graphs, 
%Our model builds on the work of \textcite{chandrasekhar2018distributed}. They propose a biologically feasible distributed algorithm that could plausibly describe how arboreal turtle ants maintain trail networks, finding alternative paths to circumvent broken links. They also investigate various local decision rules that ants may use for selecting edges to traverse. Among the decision rules considered, they found that the linear decision rule is the most likely to explain the choices ants made in field observations. However, they notice that with the linear decision rule, the dynamics fail to converge to a single consensus path, contradicting field observations where ants regularly converge to a single path. However, we show that under the forces of increasing flow or leakage (which were not considered in \autocite{chandrasekhar2018distributed}), with the linear decision rule, the dynamics always converge to a path. Therefore, our results suggest plausible ways in which these ants can use the linear decision rule and still converge to a path.

%[paraphrasing MC: what results are possible for general graphs? We showed this for a simple 2-part network. For more general situations we know from simulations that similar results seem to be true, but this raises a new question...]


%We demonstrate that leakage at vertices and increasing flow results in convergence  to the minimum leakage and the shortest path respectively. This holds for the linear decision rule where the flow divides in proportion to the pheromone level. We further show that the bidirectional nature of flow is necessary for convergence to such paths. 

%We then investigate non-linear decision rules. We consider a reasonably general family of decision rules, and show that the linear decision rule is its unique member with guaranteed convergence to the shortest or the minimum leakage path. Does it mean that the usefulness of the forces of increasing flow and leakage is only restricted to the linear decision rule? Through simulation with various non-linear decision rules, we observe that for most graph instances, the path found in the presence of these forces has length (respectively leakage) smaller than or equal to the length (respectively leakage) of the path found in their absence. This suggests that the usefulness of increasing flow and leakage in finding desirable paths is not limited to the linear decision rule.


%We believe that these results are interesting both from an algorithmic and a biological point of view. From an algorithmic standpoint, these results contribute to the rich theory of reinforced random walks \autocite{diaconis1980finetti,davis1990reinforced,pemantle2007survey}, and might be applicable to application domains involving swarm computing and molecular robots \autocite{lund2010molecular, brambilla2013swarm, werfel2014designing, hecker2015beyond} . From a biological point of view, these results provide plausible explanations for field experiments, and open up new avenues for further investigation. \autocite{chandrasekhar2019better} noticed in field observations that turtle ants favour paths which minimize the probability of getting lost. These result suggests a plausible way in which ants converge to such paths. Our result on increasing flow suggests that at least in principle, ants can obtain information about path length just by changing their flow rate. It would be fascinating to explore experimentally whether certain ant species actually increase their flow rates to find short paths.
%Results interesting from both biological, algorithmic and mathematical pov.

%Open problems: 

==> other_stuff.tex <==
\section{Proof idea for the symmetric case}
Here we study the symmetric case where we make the following assumptions.


\paragraph{Assumptions:} For intuition purposes we make the following assumptions.
\begin{itemize}
    \item Let the initial pheromone levels on all the edges be the same. \item Let $\ell(t)=r(t)$ and define $p(t)\defeq \ell(t)=r(t)$.
\end{itemize}

\subsection{Case $n=m$}
Here we assume that the path length of both the top and the bottom path are the same, that is we assume $n=m$. For this special setting the update rule of our model can be written as follows,
\begin{equation}
 f_{BD}(t) = \delta \left(f_{BD}(t-1) + p_{BD}(t-1) + \alpha p_{BD}(t-n)\right)~,
\end{equation}
 where $\pbd(t)$ denotes the flow entering the edge $(B,D)$ at time $t$ from $B$. Similarly define,
 \begin{equation}
 f_{BC}(t) = \delta \left(f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)\right)~,
\end{equation}
 where $\pbc(t)$ denotes the flow entering the edge $(B,C)$ at time $t$ from $B$.

Define for any time $t$,
\begin{equation}
    r_{t}\defeq \frac{\fbd(t)}{\fbc(t)}~.
\end{equation}

\begin{defn}
At time $t >n$, we say the system is in \emph{monotonically converging plus} (MC+) state if the following two conditions hold,
\begin{enumerate}
    \item The ratios of flow in the last $n$ time steps is non decreasing, that is, $r_{t-n+1}\leq \cdots\leq r_{t}$.
    \item At time $t$, $r_{t} \leq \frac{\alpha}{\beta}r_{t-n+1}$.
\end{enumerate}
\end{defn}

\begin{lemma}\label{lem:MC}
For any time $t>n+1$, if the system is in MC+ state at time $t-1$ then it is also at time $t$.
\end{lemma}
\begin{proof}
To prove the lemma all we need is to show that, $$r_{t} \leq \frac{\alpha}{\beta}r_{t-n+1}\text{ and }r_{t-1} \leq r_{t}~.$$ 
To prove the lemma, we first simplify the expression for $r_{t}$.
\begin{align}
    r_t&=\frac{f_{BD}(t-1) + p_{BD}(t-1) + \alpha p_{BD}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)},\nonumber\\
    &=\frac{r_{t-1}f_{BC}(t-1) + r_{t-1}p_{BC}(t-1) + \frac{\alpha}{\beta}r_{t-n} \beta p_{BC}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)}\label{eq:rt}~.
\end{align}
As the system is in MC+ state at time $t-1$ we have $\frac{\alpha}{\beta}r_{t-n} \geq r_{t-1}$ and substituting it back in the last term of the above Equation (\ref{eq:rt}) we get,
$$r_{t}\geq r_{t-1}~.$$
Further using the inequality $\frac{\alpha}{\beta}r_{t-n} \geq r_{t-1}$ and substituting it in the first two terms of the Equation (\ref{eq:rt}) we get,
$$r_{t} \leq \frac{\alpha}{\beta}r_{t-n} \leq \frac{\alpha}{\beta}r_{t-n+1}~.$$
In the last inequality we used the non-decreasing property of the MC+ state at time $t-1$.
\end{proof}


\begin{lemma}\label{lem:pbound}
For all $t\geq 0$, $\pmin\leq p(t)\leq \pmax$ and edges $e \in \{(B,C),(B,D)\}$ the following inequality holds, 
\begin{equation}
    f_{e}(t) \leq C_{p,\delta}\defeq \frac{2p}{1-\delta}~.
\end{equation}
\end{lemma}
\begin{proof}
Consider edge $e=(B,D)$, the pheromone level on edge $e$ at time $t>n$,
\begin{align}
    f_{e}(t) & = \delta \left(f_{e}(t-1) + p_{e}(t-1) + \alpha p_{e}(t-n)\right)~,\\
    & \leq \delta \left(f_{e}(t-1) + p(t) + \alpha p(t-n)\right)~,\\
    & \leq \delta \left(f_{e}(t-1) + p + \alpha p\right)~,\\
    & \leq p(1 + \alpha) \sum_{i \geq 1}\delta ^{i} \leq \frac{p(1 + \alpha)}{1-\delta} \leq \frac{2p}{1-\delta}~.
\end{align}
Similar proof also holds for edge $e=(B,C)$.
\end{proof}
In the remainder of this section we prove that single path wins.
\begin{lemma}
For any time $t>2n$, if the system is in MC state at time $t$ then,
$$\frac{f_{BD}(t')}{f_{BC}(t')} \to \infty \text{ as }t' \to \infty~.$$
\end{lemma}
\begin{proof}
\kiran{This is the sketch of the proof, need to finish it.}
$$r_{t-1}\leq (1+\epsilon/2)r_{t-n}$$
\begin{align}
    r_t&=\frac{r_{t-1}f_{BC}(t-1) + r_{t-1}p_{BC}(t-1) + ({1+\epsilon_1})r_{t-1} \beta p_{BC}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)}\label{eq:rt}~,\\
    &\geq r_{t-1} + \frac{\epsilon_1 \beta r_{t-1} p_{BC}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)}
\end{align}
Need lower bound for the following,
\begin{align}
    \frac{p_{BC}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)}\geq \frac{p_{BC}(t-n)}{2 C_{p,\delta} + \beta p_{BC}(t-n)} \geq ,\\
\end{align}

$$f_{BC}(t-1),p_{BC}(t-1) \leq \frac{\alpha}{\beta}^np_{BC}(t-n)~.$$

$$f_{BC}(t-1)=\frac{1}{p(t-1)}p_{BC}(t-1) (f_{BC}(t-1)+f_{BD}(t-1))\leq \frac{1}{p(t-1)}p_{BC}(t-1) (2C_{p,\delta})~.$$
\end{proof}


\subsection{Case $n \neq m$}
Here we study the case where $n\neq m$.
\begin{equation}
 f_{BD}(t) = \delta \left(f_{BD}(t-1) + p_{BD}(t-1) + \alpha p_{BD}(t-n)\right)~,
\end{equation}
where $\pbd(t)$ denotes the flow entering the edge $(B,D)$ at time $t$ from $B$. Similarly define,
 \begin{equation}
 f_{BC}(t) = \delta \left(f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-m)\right)~,
\end{equation}
where $\pbc(t)$ denotes the flow entering the edge $(B,C)$ at time $t$ from $B$.

Here we define the following notations,
\begin{equation}
    r_{t}\defeq \frac{\fbd(t)}{\fbc(t)} \text{ and } s_{t-n,t-m}=\frac{p_{BD}(t-n)}{p_{BC}(t-m)}~.
\end{equation}
$$\frac{p_{BD}(t-n)}{p_{BC}(t-m)} \leq \frac{p_{BD}(t-n+1)}{p_{BC}(t-m+1)} \Leftrightarrow \frac{p_{BC}(t-m+1)}{p_{BC}(t-m)} \leq \frac{p_{BD}(t-n+1)}{p_{BD}(t-n)}~.$$

\begin{equation}
    p_{BD}(t-n+1)=p\cdot \frac{f_{BD}(t-n+1)}{f_{BD}(t-n+1)+f_{BC}(t-n+1)}=p\cdot \frac{r_{t-n+1}}{1+r_{t-n+1}} \geq p\cdot \frac{r_{t-n}}{1+r_{t-n}}
\end{equation}

$$\frac{f_{BD}(t)}{f_{BC}(t)}=\frac{f'_{BD}(t+n-m)}{f'_{BC}(t)}$$

\begin{defn}
At time $t >\max(n,m)$, we say the system is in \emph{monotonically converging plus} (MC+) state if the following two conditions hold,
\begin{enumerate}
    \item The ratios of flow in the last $\max(n,m)$ time steps is non decreasing, that is, $r_{t-\max(n,m)}\leq \cdots\leq r_{t}$.
    \item At time $t$, $r_{t} \leq \frac{\alpha}{\beta}s_{t-n+1,t-m+1}$.
    \item At time $t$, $s_{t-n+1,t-m+1} \leq s_{t-n+2,t-m+2}$.
\end{enumerate}
\end{defn}


\begin{lemma}\label{lem:MC}
For any time $t>n+1$, if the system is in MC+ state at time $t-1$ then it is also at time $t$.
\end{lemma}
\begin{proof}
To prove the lemma all we need is to show that, $$r_{t} \leq \frac{\alpha}{\beta}s_{t-n+1,t-m+1},\quad  s_{t-n+1,t-m+1} \leq s_{t-n+2,t-m+2},\quad \text{ and }r_{t-1} \leq r_{t}~.$$ 
To prove the lemma, we first simplify the expression for $r_{t}$.
\begin{align}
    r_t&=\frac{f_{BD}(t-1) + p_{BD}(t-1) + \alpha p_{BD}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-m)},\nonumber\\
    &=\frac{r_{t-1}f_{BC}(t-1) + r_{t-1}p_{BC}(t-1) + \frac{\alpha}{\beta}s_{t-n,t-m} \beta p_{BC}(t-n)}{f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-m)}\label{eq:rt}~.
\end{align}
As the system is in MC+ state at time $t-1$ we have $\frac{\alpha}{\beta}s_{t-n,t-m} \geq r_{t-1}$ and substituting it back in the last term of the above Equation (\ref{eq:rt}) we get,
$$r_{t}\geq r_{t-1}~.$$
Further using the inequality $\frac{\alpha}{\beta}s_{t-n,t-m} \geq r_{t-1}$ and substituting it in the first two terms of the Equation (\ref{eq:rt}) we get,
$$r_{t} \leq \frac{\alpha}{\beta}s_{t-n,t-m} \leq \frac{\alpha}{\beta}s_{t-n+1,t-m+1}~.$$
All that remains is to prove the following inequality,
$$s_{t-n+1,t-m+1} \leq s_{t-n+2,t-m+2}~.$$
For fixed flow, the above expression can be simplified as follows,
\begin{align}
    s_{t-n+1,t-m+1} \leq s_{t-n+2,t-m+2}& \Leftrightarrow\frac{p_{BD}(t-n+1)}{p_{BC}(t-m+1)}\leq \frac{p_{BD}(t-n+2)}{p_{BC}(t-m+2)}~,\\
    &\Leftrightarrow\frac{p_{BD}(t-n+1)}{p_{BD}(t-n+2)}\leq \frac{p_{BC}(t-m+1)}{p_{BC}(t-m+2)}~,\\
    &\Leftrightarrow\frac{\frac{f_{BD}(t-n+1)}{f_{BD}(t-n+1)+f_{BC}(t-n+1)}}{\frac{f_{BD}(t-n+2)}{f_{BD}(t-n+2)+f_{BC}(t-n+2)}}\leq \frac{\frac{f_{BC}(t-m+1)}{f_{BD}(t-m+1)+f_{BC}(t-m+1)}}{\frac{f_{BC}(t-m+2)}{f_{BD}(t-m+2)+f_{BC}(t-m+2)}}~,\\
    &\Leftrightarrow \frac{\frac{r_{t-n+1}}{1+r_{t-n+1}}}{\frac{r_{t-n+2}}{1+r_{t-n+2}}} \leq \frac{\frac{1}{1+r_{t-m+1}}}{\frac{1}{1+r_{t-m+2}}}
    \Leftrightarrow \frac{r_{t-n+1}}{r_{t-n+2}} \cdot \frac{1+r_{t-n+2}}{1+r_{t-n+1}} \leq \frac{1+r_{t-m+2}}{1+r_{t-m+1}}~.
\end{align}

Therefore all we need to show is that,
$$\frac{r_{t-n+1}}{r_{t-n+2}} \cdot \frac{1+r_{t-n+2}}{1+r_{t-n+1}} \leq \frac{1+r_{t-m+2}}{1+r_{t-m+1}}~.$$
Now note that,
\begin{align*}
    \frac{r_{t-n+1}}{r_{t-n+2}} \cdot \frac{1+r_{t-n+2}}{1+r_{t-n+1}} & = \frac{1+\frac{1}{r_{t-n+2}}}{1+\frac{1}{r_{t-n+1}}}
     \leq 1  \leq \frac{1+r_{t-m+2}}{1+r_{t-m+1}}~.
\end{align*}
In the third and fourth inequality above we used $r_{t-n+1} \leq r_{t-n+2}$ and $r_{t-m+1} \leq r_{t-m+2}$ respectively.
\end{proof}

\section{Unravelling and alternate proof}
Here we assume that the path length of both the top and the bottom path are the same, that is we assume $n=m$. For this special setting the update rule of our model can be written as follows,
\begin{equation}
 f_{BD}(t) = \delta \left(f_{BD}(t-1) + p_{BD}(t-1) + \alpha p_{BD}(t-n)\right)~,
\end{equation}
 where $\pbd(t)$ denotes the flow entering the edge $(B,D)$ at time $t$ from $B$. Similarly define,
 \begin{equation}
 f_{BC}(t) = \delta \left(f_{BC}(t-1) + p_{BC}(t-1) + \beta p_{BC}(t-n)\right)~,
\end{equation}
 where $\pbc(t)$ denotes the flow entering the edge $(B,C)$ at time $t$ from $B$.
 
\begin{defn}
At time $t >2n$, we say the system is in \emph{monotonically converging} (MC) state if the following two conditions hold,
\begin{enumerate}
    \item The ratios of flow in the last $2n$ time steps $\{\frac{p_{BD}(t - 2n + 1)}{p_{BC}(t - 2n + 1)}, \cdots, \frac{p_{BD}(t - 1)}{p_{BC}(t -  1)} \}$ is increasing.
    \item The ratios in the last 2n time steps are increasing but not too fast, i.e. $\frac{f_{BD}(t-i)}{f_{BC}(t-i)} \leq \frac{\alpha f_{BD}(t-i - n+1)}{\beta f_{BC}(t-i-n+1)} $ for all $2n \geq i \geq 1$.
\end{enumerate}
\end{defn}

\begin{lemma}\label{lem:MC}
For any time $t>2n$, if the system is in MC state then it is also at time $t+1$.
\end{lemma}
\begin{proof}
To prove the lemma all we need is to show that, $$\frac{f_{BD}(t)}{f_{BC}(t)} \leq \frac{\alpha f_{BD}(t-n+1)}{\beta f_{BC}(t-n+1)} \text{ and }\frac{p_{BD}(t )}{p_{BC}(t )} \leq \frac{p_{BD}(t + 1)}{p_{BC}(t +  1)}~.$$ 
As the first inequality here implies the second, so we just need to prove the former.
%We basically want to show that if the ratio of pheromones has been increasing slowly over the last 2n time steps, it will do so in the next time step as well.
Unrolling $f_{BD}(t)$ and $f_{BC}(t)$ we get,
\begin{equation}
f_{BD}(t) = \delta^n f_{BD}(t-n) + \sum_{i = 1}^n \delta^i p_{BD}(t-i) + \alpha \sum_{i=1}^n \delta^i p_{BD}(t-n-i+1)~.
\end{equation}
\begin{equation}
f_{BC}(t) = \delta^n f_{BC}(t-n) + \sum_{i = 1}^n \delta^i p_{BC}(t-i) + \beta \sum_{i=1}^n \delta^i p_{BC}(t-n-i+1) ~.
\end{equation}
As the system is in MC state at time $t$ we get,
$$\frac{p_{BD}(t-i)}{p_{BC}(t-i)} = \frac{f_{BD}(t-i)}{f_{BC}(t-i)} \leq \frac{\alpha f_{BD}(t-i - n+1)}{\beta f_{BC}(t-i-n+1)} \leq \frac{\alpha f_{BD}(t-n)}{\beta f_{BC}(t-n)}~.$$
Also,
$$\frac{\alpha p_{BD}(t-n-i+1)}{\beta  p_{BC}(t-n-i+1)} = \frac{\alpha  f_{BD}(t-n-i+1)}{\beta f_{BC}(t-n-i+1)} \leq \frac{\alpha  f_{BD}(t-n)}{\beta f_{BC}(t-n)}~.$$
Combining these expressions, we can get
$$\frac{f_{BD}(t)}{f_{BC}(t)} \leq \frac{\alpha  f_{BD}(t-n)}{\beta f_{BC}(t-n)} \leq \frac{\alpha  f_{BD}(t-n+1)}{\beta f_{BC}(t-n+1)}~,$$ and we conclude the proof.
\end{proof}




Define for any time $t$,
\begin{equation}
    r_{t}\defeq \frac{\fbd(t)}{\fbc(t)}~.
\end{equation}



\begin{lemma}\label{lem:pbound}
For all $t\geq 0$, $\pmin\leq p(t)\leq \pmax$ and edges $e \in \{(B,C),(B,D)\}$ the following inequality holds, 
\begin{equation}
    f_{e}(t) \leq C_{p,\delta}\defeq \frac{2p}{1-\delta}~.
\end{equation}
\end{lemma}
\begin{proof}
Consider edge $e=(B,D)$, the pheromone level on edge $e$ at time $t>n$,
\begin{align}
    f_{e}(t) & = \delta \left(f_{e}(t-1) + p_{e}(t-1) + \alpha p_{e}(t-n)\right)~,\\
    & \leq \delta \left(f_{e}(t-1) + p(t) + \alpha p(t-n)\right)~,\\
    & \leq \delta \left(f_{e}(t-1) + p + \alpha p\right)~,\\
    & \leq p(1 + \alpha) \sum_{i \geq 1}\delta ^{i} \leq \frac{p(1 + \alpha)}{1-\delta} \leq \frac{2p}{1-\delta}~.
\end{align}
Similar proof also holds for edge $e=(B,C)$.
\end{proof}
In the remainder of this section we prove that single path wins.
\begin{lemma}
For any time $t>2n$, if the system is in MC state at time $t$ then,
$$\frac{f_{BD}(t')}{f_{BC}(t')} \to \infty \text{ as }t' \to \infty~.$$
\end{lemma}
\begin{proof}
For any $t'\geq 0$ define, $r_{t'}\defeq \frac{f_{BD}(t')}{f_{BC}(t')}=\frac{p_{BD}(t')}{p_{BC}(t')}$. Since the system is in MC state at time $t$, by Lemma~\ref{lem:MC} we know that it is in MC state for all $t' \geq t$. For any $t'>t+2n$, in the remainder of the proof we show that at least one of the following two conditions hold,
\begin{enumerate}
    \item Either $$\frac{\alpha}{\beta}r_{t'-n}\leq  r_{t'-1}+\frac{2\epsilon(2+r_{t}) r_{t'-n}}{\pmin}~.$$
    \item Else, $$r_{t'} \geq r_{t'-1}+\frac{\delta \epsilon}{C_{p,\delta}}~.$$
\end{enumerate}
%The above result immediately implies the lemma because we make a non-trivial progress in every $n$ steps, that is, if the first condition holds then we have,
%$$\frac{f_{BD}(t')}{f_{BC}(t')}\geq \frac{f_{BD}(t'-1)}{f_{BC}(t'-1)}>(1+\epsilon_1)\frac{f_{BD}(t'-n)}{f_{BC}(t'-n)}~.$$
%Else we know that the second condition holds, therefore,
%$$\frac{f_{BD}(t')}{f_{BC}(t')}>(1+\epsilon_2)\frac{f_{BD}(t'-1)}{f_{BC}(t'-1)} \geq (1+\epsilon_2)\frac{f_{BD}(t'-n)}{f_{BC}(t'-n)}.$$
Now define $U\defeq \frac{2(2+r_{t}) }{\pmin}$ and note that it is a fixed constant that doesn't depend on $t'$. Now the first condition above can be equivalently written as,
\begin{equation}
    r_{t'-1} \geq r_{t'-n} + \left(\frac{\alpha-\beta}{\beta}-\epsilon U\right)r_{t'-n}
\end{equation}
We now choose $\epsilon$ such that, 
\begin{equation}
    \left(\frac{\alpha-\beta}{\beta}-\epsilon U\right)r_{t'-n}=\frac{\delta \epsilon}{C_{p,\delta}} \Leftrightarrow \epsilon = \frac{\alpha-\beta}{\beta} \left(\frac{\delta }{C_{p,\delta}r_{t'-n}}+U\right)^{-1}~,
\end{equation}
As the system is in MC state the ratio $r_{t'}$ is non-decreasing we have $r_{t'}\geq r_{t'-1}$, $r_{t'-1}\geq r_{t'-n}$ and for the above choice of $\epsilon$ we get,
$$r_{t'}-r_{t'-n}>\frac{\delta \epsilon}{C_{p,\delta}}\geq \frac{\delta }{C_{p,\delta}}\frac{\alpha-\beta}{\beta} \left(\frac{\delta }{C_{p,\delta}r_{t'-n}}+U\right)^{-1} \geq \frac{\delta }{C_{p,\delta}}\frac{\alpha-\beta}{\beta} \left(\frac{\delta }{C_{p,\delta}r_{t}}+U\right)^{-1}.$$
The amount of increase in $n$ time steps in a fixed constant independent of $t'$ and the above inequality immediately implies the lemma and all that remains is to prove the conditions mentioned at the start of the lemma.

Suppose condition 1 holds, then we are done. Therefore without loss of generality we assume,

Since,
\begin{align}
    r_{t'-1}+\frac{\epsilon}{\beta p_{BC}(t'-n)} & \leq r_{t'-1}+\frac{\epsilon r_{t'-n}}{\beta p_{BD}(t'-n)} \leq r_{t'-1}+\frac{\epsilon r_{t'-n}}{\beta p_{BD}(t'-n)}\leq r_{t'-1}+\frac{2\epsilon(2+r_{t}) r_{t'-n}}{\pmin},\\
\end{align}
Suppose the condition 1 does not hold then we get the following inequality due to above expression,
$$\frac{\alpha}{\beta}r_{t'-n}\geq  r_{t'-1}+\frac{2\epsilon(2+r_{t}) r_{t'-n}}{\pmin} \implies \frac{\alpha}{\beta}r_{t'-n}\geq r_{t'-1}+\frac{\epsilon}{\beta p_{BC}(t'-n)}~.$$
The above inequality immediately implies the following,
\begin{align}
r_{t'} &= \frac{\delta \left(f_{BD}(t'-1) + p_{BD}(t'-1) + \alpha p_{BD}(t'-n)\right)}{\delta \left(f_{BC}(t'-1) + p_{BC}(t'-1) + \beta p_{BC}(t'-n)\right)}~,\\
&=\frac{r_{t'-1}f_{BC}(t'-1) + r_{t'-1}p_{BC}(t'-1) + (\frac{\alpha}{\beta}r_{t-n})\beta p_{BC}(t'-n)}{f_{BC}(t'-1) + p_{BC}(t'-1) + \beta p_{BC}(t'-n)}~,\\
&\geq \frac{r_{t'-1}f_{BC}(t'-1) + r_{t'-1}p_{BC}(t'-1) + (r_{t'-1}+\frac{\epsilon}{\beta p_{BC}(t'-n)})\beta p_{BC}(t'-n)}{f_{BC}(t'-1) + p_{BC}(t'-1) + \beta p_{BC}(t'-n)}~,\\
&\geq r_{t'-1}+\frac{\epsilon}{f_{BC}(t'-1) + p_{BC}(t'-1) + \beta p_{BC}(t'-n)}~,\\
& = r_{t'-1}+\frac{\delta \epsilon}{f_{BC}(t')}\geq r_{t'-1}+\frac{\delta \epsilon}{C_{p,\delta}}~.\\
\end{align}
In the last inequality we used Lemma \ref{lem:pbound}
\end{proof}


==> preamble.tex <==
\makeatletter



\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}


% -- Options

\RequirePackage{options}

\options{
	/opts/.new family,
	/opts/colors/.new toggle=true,
	/opts/fonts/.new toggle=true,
	/opts/math/.new toggle=true,
	/opts/theorems/.new toggle=true,
	/opts/macros/.new toggle=true,
	/opts/graphics/.new toggle=true,
	/opts/tools/.new toggle=true,
	/opts/typesetting/.new toggle=true,
	/opts/biblio/.new toggle=true
}
\options{/opts}

\providetoggle{presentation}
\@ifclassloaded{beamer}{\toggletrue{presentation}}{\togglefalse{presentation}}

% -- Packages
% \usepackage{natbib}
% \bibliographystyle{unsrtnat}
\usepackage[
backend=biber,
style=alphabetic,
citestyle= alphabetic,
maxbibnames = 99,
maxcitenames = 2,
url = false
]{biblatex}


\addbibresource{references.bib}

\iftoggle{/opts/math}{
	\RequirePackage{amsmath}
	\RequirePackage{amssymb}
	\RequirePackage{bm}
	\RequirePackage{dsfont}
	\RequirePackage{mathtools}
}{}

\iftoggle{/opts/theorems}{
	\RequirePackage{amsthm}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikz}
	\RequirePackage{tikz-3dplot}
	\RequirePackage{tcolorbox}
	\RequirePackage{pgfplots}
	\RequirePackage{tcolorbox}
	\pgfplotsset{compat=newest}
}{}

\iftoggle{/opts/tools}{
	\RequirePackage[ruled]{algorithm2e}
	\RequirePackage{datatool}
	\RequirePackage[super]{nth}
	\RequirePackage{scalerel}
	\iftoggle{presentation}{}{
		\RequirePackage[shortlabels]{enumitem}
	}
}{}

\iftoggle{/opts/fonts}{
	\iftoggle{presentation}{}{
		\RequirePackage[sc]{mathpazo}
	}
}{}

\iftoggle{/opts/biblio}{
	\iftoggle{presentation}{}{
		\RequirePackage[backend=biber, style=alphabetic, maxbibnames=99, maxcitenames=2, url=false]{biblatex}
	}
}

\iftoggle{/opts/colors}{
	\newcommand{\declarecolor}[2]{\@ifundefined{\string\color@#1}{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}{}}
	\declarecolor{Black}{0, 0, 0}
	\declarecolor{White}{255, 255, 255}
	\declarecolor{Gray}{127, 127, 127}
	\declarecolor{LightGray}{216, 216, 216}
	\declarecolor{Orange}{237, 125, 49}
	\declarecolor{LightOrange}{251,229, 214}
	\declarecolor{Yellow}{255, 192, 0}
	\declarecolor{LightYellow}{255, 242, 200}
	\declarecolor{Blue}{91, 155, 213}
	\declarecolor{LightBlue}{222, 235, 247}
	\declarecolor{Green}{112, 173, 71}
	\declarecolor{LightGreen}{226, 240, 217}
	\declarecolor{Navy}{68, 114, 196}
	\declarecolor{LightNavy}{218, 227, 243}
	
	\newcommand{\declareperson}[1]{%
		\expandafter\newcommand\csname#1\endcsname[1]{\textcolor{Orange}{#1: ##1}}%
	}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikzsymbols}
	
	\usetikzlibrary{decorations}
	\usetikzlibrary{decorations.pathreplacing}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{fit}
	\usetikzlibrary{intersections}
	\usetikzlibrary{matrix}
	\usetikzlibrary{overlay-beamer-styles}
	\usetikzlibrary{patterns}
	\usetikzlibrary{shapes}
	\usetikzlibrary{tikzmark}
	\usetikzlibrary{hobby}
	
	\usepgflibrary{arrows.meta}
	
	\tcbuselibrary{skins}
	\tcbuselibrary{raster}
	
	\usepgfplotslibrary{patchplots}
		
	\pgfdeclarelayer{background}
	\pgfdeclarelayer{foreground}
	\pgfsetlayers{background,main,foreground}
	\tikzstyle{na}=[baseline=-0.5ex]
	\tikzset{onslide/.code args={<#1>#2}{%
	  \only<#1>{\pgfkeysalso{#2}}
	}}
	\tikzset{temporal/.code args={<#1>#2#3#4}{%
	  \temporal<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}{\pgfkeysalso{#4}}
	}}
		
	\pgfplotsset{colormap={WhiteOrange}{
		color=(White)
		color=(Orange)
	}}
	\pgfplotsset{colormap={NavyOrange}{
		color=(LightNavy)
		color=(Orange)
	}}
	\pgfplotsset{colormap={WhiteNavy}{
		color=(White)
		color=(Navy)
	}}
	\pgfplotsset{colormap={WhiteBlack}{
		color=(White)
		color=(Black)
	}}
		
	\newcommand*{\Pic}[2][]{\begin{tikzpicture}\pic[#1]{#2};\end{tikzpicture}}
	\newcommand*{\sPic}[2]{\scalebox{#1}{\Pic{#2}}}
	\newcommand*{\cPic}[2][]{\begin{center}\Pic[#1]{#2}\end{center}}
	
	\newcommand{\rounded}[2][0.7ex]{%
		\begin{tikzpicture}
			\node[inner sep=0ex, draw=White, line width=0ex, opacity=0.] (a) {#2};
			\clip[rounded corners=#1] (a.south west) rectangle (a.north east);
			\node[inner sep=0ex] (a) {#2};
		\end{tikzpicture}%
	}
	
	\newcommand*{\tnode}[2]{\tikzmarknode{#1}{#2}}
}{}

\iftoggle{/opts/typesetting}{
	\iftoggle{presentation}{
	}{
		\RequirePackage{microtype}
		\RequirePackage{parskip}
		\RequirePackage{fullpage}
	}
	\RequirePackage{hyperref}
	\RequirePackage[capitalize, nameinlink]{cleveref}
	
	\iftoggle{/opts/colors}{
		\hypersetup{
			colorlinks=true,
			pdfpagemode=UseNone,
			citecolor=Blue,
			linkcolor=Black,
			urlcolor=Blue
		}
	}{}
}{}

\iftoggle{/opts/theorems}{
	\iftoggle{presentation}{}{
		\theoremstyle{plain}
		\newtheorem{theorem}{Theorem}
		\newtheorem*{theorem*}{Theorem}
		\newtheorem{lemma}{Lemma}
		\newtheorem{corollary}{Corollary}
		\newtheorem{proposition}{Proposition}
		\newtheorem*{proposition*}{Proposition}
		\newtheorem{fact}{Fact}
		\newtheorem{conjecture}{Conjecture}
		\newtheorem*{conjecture*}{Conjecture}
		
		\theoremstyle{definition}
		\newtheorem{definition}{Definition}
		
		\theoremstyle{remark}
		\newtheorem{remark}{Remark}
		\newtheorem{example}{Example}
	}
}{}

\iftoggle{/opts/macros}{
	\providecommand{\given}{}
	\newcommand\GivenSymbol[1][]{%
		\nonscript\:#1\vert%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\newcommand{\declaredelims}[3]{%
		\expandafter\DeclarePairedDelimiterX\csname#1\endcsname[1]{#2}{#3}{\renewcommand\given{\GivenSymbol[\delimsize]}##1}%
	}
	
	\declaredelims{set}\{\}
	\declaredelims{card}\lvert\rvert
	\declaredelims{abs}\lvert\rvert
	\declaredelims{norm}\lVert\rVert
	\declaredelims{dotp}\langle\rangle
	\declaredelims{tuple}\lparen\rparen
	\declaredelims{parens}\lparen\rparen
	\declaredelims{bracks}\lbrack\rbrack
	
	\newcommand{\declarenameddelims}[4]{%
		\expandafter\DeclarePairedDelimiterXPP\csname#1\endcsname[1]{#2}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}##1}%
		\expandafter\DeclarePairedDelimiterXPP\csname#1X\endcsname[2]{#2_{##1}}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}##2}%
	}
	
	
	\let\Pr\relax
	\declarenameddelims{Pr}{\mathbb{P}}\lbrack\rbrack
	\declarenameddelims{Ex}{\mathbb{E}}\lbrack\rbrack
	
	\newcommand*{\eval}[1]{\left.#1\right\rvert}
	
	\iftoggle{presentation}{%
		\newcommand*{\mathdouble}[1]{\mathds{#1}}%
	}{%
		\newcommand*{\mathdouble}[1]{\mathbb{#1}}%
	}
	
	\let\Q\relax
	\newcommand*{\Q}{{\mathdouble{Q}}}
	\let\N\relax
	\newcommand*{\N}{{\mathdouble{N}}}
	\let\Z\relax
	\newcommand*{\Z}{{\mathdouble{Z}}}
	\let\R\relax
	\newcommand*{\R}{{\mathdouble{R}}}
	\let\C\relax
	\newcommand*{\C}{{\mathdouble{C}}}
	\let\1\relax
	\newcommand*{\1}{{\mathds{1}}}
	\let\l\relax
	\newcommand*{\l}{{\ell}}
	
	\let\poly\relax
	\DeclareMathOperator{\poly}{poly}
	\DeclareMathOperator{\supp}{supp}
	\DeclareMathOperator{\conv}{conv}
	\DeclareMathOperator{\rank}{rank}
	\let\Im\relax
	\DeclareMathOperator{\Im}{Im}
	\let\Re\relax
	\DeclareMathOperator{\Re}{Re}
}{}
\makeatother

\usepackage{thmtools}
\declaretheorem[name=Theorem,numberwithin=section]{thm}
\declaretheorem[name=Claim,numberlike=thm]{claim}
\declaretheorem[name=Claim,numberlike=thm]{clm}
\declaretheorem[name=Corollary,numberlike=thm]{cor}
\declaretheorem[name=Definition,numberlike=thm,style=definition]{defn}
\declaretheorem[name=Proposition,numberlike=theorem]{prop}
%\declaretheorem[name=Fact,numberlike=thm,style=definition]{fact}



\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newcommand{\fflow}[1]{ f_{\overset{\rightarrow}{#1}}}
\newcommand{\bflow}[1]{ f_{\overset{\leftarrow}{#1}}}

\newcommand{\nfflow}[1]{\overline{f}_{\overset{\rightarrow}{#1}}}
\newcommand{\nbflow}[1]{\overline{f}_{\overset{\leftarrow}{#1}}}

\newcommand{\nfp}[1]{\overline{p}_{\overset{\rightarrow}{#1}}}
\newcommand{\nbp}[1]{\overline{p}_{\overset{\leftarrow}{#1}}}

\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{multirow}


\newcommand{\fbc}{{f_{BC}}}
\newcommand{\fbd}{{f_{BD}}}
\newcommand{\pbc}{{p_{BC}}}
\newcommand{\pbd}{{p_{BD}}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}
\newcommand{\pmax}{p_{\max}}
\newcommand{\pmin}{p_{\min}}
\newcommand{\setflb}{\mathcal{F}}
\newcommand{\rmin}{r_{\text{min}}}
\newcommand{\epsp}{\epsilon'}

==> proof_ideas_long.tex <==
\section{Proof Ideas}
\label{sec:proof_overview}
In this section, we describe  the proof ideas for our results. Complete proofs are given in Appendix.
\subsection{Linear Decision Rule with Leakage}
For a graph consisting of two parallel paths $P_1$ and $P_2$, with $l_{P_1} < l_{P_2}$, we show in \Cref{thm:ub-leakage} that the dynamics converges to the path $P_1$ when the incoming forward and backward flow values are fixed. Less leakage on $P_1$ ensures that relatively more pheromone accumulates on it with time. 

Let $s_1$ and $s_2$ be the neighboring vertices of $s$, and $d_1$ and $d_2$ be the neighboring vertices of $d$, on path $P_1$ and $P_2$ respectively. Note that only the pheromone level on edges $(s, s_1), (s, s_2), (d_1, d), (d_2, d)$ affect the dynamics for this graph.  To get some intuition, it is instructive to consider the ratio of pheromone levels on $(s, s_1)$ and $(s, s_2)$ at time $(t+1)$:
\begin{align}
    \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)} &= \frac{\delta(p_{ss_1}(t) + \fflow{ss_1}(t)  + \bflow{ss_1}(t))}{\delta(p_{ss_2}(t) + \fflow{ss_2}(t)  + \bflow{ss_2}(t))}\\
    &= \frac{p_{ss_1}(t) + \fflow{ss_1}(t)  + (1 - l_{P_1})\bflow{d_1d}(t- len_{P_1}+1)}{p_{ss_2}(t ) + \fflow{ss_2}(t)  + (1 - l_{P_2})\bflow{d_2d}(t - len_{P_2}+1)}
\end{align}
Here, $len_{P_1}$ and $len_{P_2}$ represent the lengths of path $P_1$ and $P_2$. Now, note that the forward flow at $s$ divides itself in the ratio of pheromone at $(s, s_1)$ and $(s, s_2)$, that is, 
$\frac{\fflow{ss_1}(t)}{\fflow{ss_2}(t)} = \frac{p_{ss_1}(t)}{p_{ss_2}(t)}$. Therefore, 
the forward flows $\fflow{ss_1}$ and $\fflow{ss_2}$ do not affect the ratio of the pheromone levels $\frac{p_{ss_1}}{p_{ss_2}}$. The relationship between $\frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)}$ and $\frac{p_{ss_1}(t)}{p_{ss_2}(t)}$ is governed by the backward flow coming from $d$. Since leakage $l_{P_1} < l_{P_2}$, the $(1 - l_{P_1})$ and $(1 - l_{P_2})$ terms would ensure $\frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)} > \frac{p_{ss_1}(t)}{p_{ss_2}(t) }$, if $\frac{\bflow{d_1d}(t- len_{P_1}+1)}{\bflow{d_2d}(t - len_{P_2}+1)} \geq \frac{p_{ss_1}(t)}{p_{ss_2}(t)}$. However, this is not true in general, and the ratio of pheromone levels $p_{ss_1}$ and $p_{ss_2}$ does not increase monotonically with time. As the lengths of the two paths can be different, directly analysing the trajectory of the ratio of pheromone level becomes tricky even for this seemingly simple case. 

To get past this hurdle, we need to carefully construct a potential function which increases monotonically with time.
Our potential function is  given by the minimum of the ratio of the pheromone levels $\frac{p_{ss_1}(t)}{p_{ss_2}(t)}$ and $\frac{p_{d_1d}(t)}{p_{d_2d}(t)}$ across the last $max(len_{P_1}, len_{P_2})$ time steps. Let $r_{ss_1}(t) \defeq \frac{p_{ss_1}(t)}{p_{ss_2}(t)}$, $r_{ss_2}(t) \defeq \frac{p_{d_1d}(t)}{p_{d_2d}(t)}$, and $L \defeq max(len_{P_1}, len_{P_2})$. Our potential function is given by 

$$r_{min}(t) \defeq min\{r_{ss_1}(t), r_{ss_1}(t-1), \cdots, r_{ss_1}(t-L+1), r_{d_1d}(t), r_{d_1d}(t-1), \cdots, r_{d_1d}(t-L+1)   \}. $$

Let the fixed incoming flows at $s$ and $d$ be given by $\fflow{s}$ and $\bflow{d}$ respectively.
From the definition, we know that $\frac{\fflow{ss_1}(t)}{\fflow{ss_2}(t)} = \frac{p_{ss_1}(t)}{p_{ss_2}(t)} = r_{ss_1}(t) \geq r_{min}(t)$. 
Further, it is not hard to see that $\bflow{d_1d}(t- len_{P_1}+1) \geq  \frac{r_{min}(t) \bflow{d} }{1+r_{min}(t)}$, and $\bflow{d_2d}(t- len_{P_2}+1) \leq  \frac{\bflow{d} }{1+r_{min}(t)}$, which implies $\frac{\bflow{d_1d}(t- len_{P_1}+1)}{\bflow{d_2d}(t- len_{P_2}+1)} \geq r_{min}(t)$. These inequalities give us
\begin{align}
   \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)} &\geq r_{min}(t)\frac{p_{ss_2}(t) + \fflow{ss_2}(t)  + (1 - l_{P_1})\bflow{d_2d}(t- len_{P_2}+1)}{p_{ss_2}(t ) + \fflow{ss_2}(t)  + (1 - l_{P_2})\bflow{d_2d}(t - len_{P_2}+1)}\\
   &> r_{min}(t)
\end{align}
where we used $l_{P_1} < l_{P_2}$ for the last inequality. This gives us $\frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)} = r_{ss_1}(t+1) > r_{min}(t)$. Similarly, we can show $r_{d_1d}(t+1) > r_{min}(t)$. This implies that $r_{min}(t)$ never decreases, and strictly increases every $L$ time steps. In \Cref{sec:appendix-ub-proofs}, we show that this increase is at least by a factor of $(1+c)$ for some constant $c > 0$. This implies the convergence of the dynamics to path $P_1$.

\subsection{Linear Decision Rule with Increasing Flow}
For a graph consisting of two parallel paths $P_1$ and $P_2$, with $len_{P_1} < len_{P_2}$, we show in \Cref{thm:ub-changing-flow} that the dynamics converges to the path $P_1$ when the incoming forward and backward flow values increase by a multiplicative or additive factor with time.
Again, consider the ratio of pheromone levels on $(s, s_1)$ and $(s, s_2)$ at time $t+1$:
\begin{align}
    \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)}
    &= \frac{p_{ss_1}(t) + \fflow{ss_1}(t)  + (1 - l_{P_1})\bflow{d_1d}(t- len_{P_1}+1)}{p_{ss_2}(t ) + \fflow{ss_2}(t)  + (1 - l_{P_2})\bflow{d_2d}(t - len_{P_2}+1)}
\end{align}
Setting leakage $l_{P_1} = l_{P_2} = 0$, and writing the backward flow in terms of normalized pheromone level, we get:
\begin{align}
    \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)}
    &= \frac{p_{ss_1}(t) + \fflow{ss_1}(t)  + \bflow{d}(t- len_{P_1}+1) \nbp{d_1d}(t - len_{P_1}+1)}{p_{ss_2}(t ) + \fflow{ss_2}(t)  + \bflow{d}(t - len_{P_2}+1)\nbp{d_2d}(t - len_{P_2}+1)}
\end{align}
For simplicity, let us assume $\bflow{d}(t) = \alpha^t$, for some $\alpha > 1$. This gives
\begin{align}
    \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)}
    &= \frac{p_{ss_1}(t) + \fflow{ss_1}(t)  + \alpha^{(t - len_{P_1}+1)} \nbp{d_1d}(t - len_{P_1}+1)}{p_{ss_2}(t ) + \fflow{ss_2}(t)  + \alpha^{(t - len_{P_2}+1)}\nbp{d_2d}(t - len_{P_2}+1)}
\end{align}
As $len_{P_1} < len_{P_2}$, we get $\alpha^{(t - len_{P_1}+1)} > \alpha^{(t - len_{P_2}+1)}$. $\alpha^{(t - len_{P_1}+1)}$ and $\alpha^{(t - len_{P_2}+1)}$ terms would ensure  $\frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1)} > \frac{p_{ss_1}(t+1)}{p_{ss_2}(t+1) }$, if $\frac{\nbp{d_1d}(t- len_{P_1}+1)}{\nbp{d_2d}(t - len_{P_2}+1)} \geq \frac{p_{ss_1}(t)}{p_{ss_2}(t)}$. However, this is not true in general, and the ratio of pheromone levels $p_{ss_1}$ and $p_{ss_2}$ does not increase monotonically. To get past this obstacle, similar to the proof for leakage with fixed flow case, we consider the potential function $r_{min}(t)$, given by the minimum of the ratio of the pheromone levels $\frac{p_{ss_1}(t)}{p_{ss_2}(t)}$ and $\frac{p_{d_1d}(t)}{p_{d_2d}(t)}$ across the last $max(len_{P_1}, len_{P_2})$ time steps. We show that this potential function never decreases and increases sufficiently every $max(len_{P_1}, len_{P_2})$ time steps. 

\subsection{ General Rules and Fundamental Limits}
Here we provide the proof sketch for all the results stated in \Cref{sec:general_rules_lb}. 

In \Cref{prop:one}, we claim that for any pheromone based rule $g \in \mathcal{G}$, bi-directional flow is necessary for convergence to the shortest or the minimum leakage path. The proof of this result is straightforward. Without loss of generality, let us assume there is one way flow from $s$ to $d$. In this case, the pheromone level on the edges incident on $s$ is only a function of their initial pheromone level and  forward flow at $s$. It does not depend on the flows and pheromone levels on the rest of the graph. Therefore, in the case of two parallel paths, for a given decision rule and initial setting of the pheromone levels, if the dynamics converges to a particular path, then they will converge to the other path if we swap the initial pheromone level on the two edges incident on $s$. Therefore, we can always set the initial pheromone levels on the edges incident on $s$, such that the dynamics does not converge to the shortest or the minimum leakage path.




Next,  we provide a proof sketch for \Cref{prop:two} and \Cref{prop:nl-incflow}. The proofs for both these results are similar and here we provide the intuition for \Cref{prop:two}. Out of the two paths, assume that the top path has smaller leakage. We would show that the dynamics is not guaranteed to converge to the top path for non-linear $g \in \setflb$. For any $g \in \setflb$, consider some $r\geq 0$  such that $g(r)\neq r$. Such an $r$ exists because $g$ is non-linear. Further, as $g$ is continuous, there exists an $\epsilon >0$ such that for all $0<s\leq \epsilon$, one of the following two conditions holds: 1) $g(r+s)< r+s$, 2) $g(r+s)>r+s$. 

Suppose $g$ is such that $g(r+s)< r+s$ for all
$0<s\leq \epsilon$.  Consider the instance where the initial normalized pheromone level and flow values on the edges of the top (minimum leakage) path are at most $r+\epsilon$ and bottom path are at least $1-r-\epsilon$. Let the forward and backward incoming flows be equal to $1$ at all times. The decision rule $g$ sends at most $r+\epsilon-c_{g,\epsilon}$ (because $g(r+\epsilon)< r+\epsilon$ and $g$ is monotone) amount of forward and backward flow on the top path and at least $1-r-\epsilon+c_{g,\epsilon}$ on the bottom path, where $c_{g,\epsilon}$ is a fixed positive constant dependent on $g$ and $\epsilon$. Now, we can choose the leakage parameter for the two paths carefully such that the normalized pheromone levels and flow levels on the top path still remain at most $r+\epsilon$ throughout the future.
Thus, the dynamics never converges to the top or the minimum leakage path. 

The intuition for the second case where $g(r+s)> r+s$ for all $0<s\leq \epsilon$ is similar. In this case we set the initial normalized pheromone level and flow values of $r+\epsilon$ on the bottom path (maximum leakage path). The rule $g$ sends at least $r+\epsilon+c_{g,\epsilon}$ (because $g(r+\epsilon)> r+\epsilon$ and $g$ is monotone) amount of flow on the bottom path. Again, with appropriately set leakage parameters, the presence of the additive term $c_{g,\epsilon}$ helps ensure that the normalized pheromone levels and the flow levels on this path never fall below $r+\epsilon$. Thus, the dynamics never converges to the minimum leakage path. 

==> simulation_figure.tex <==

\begin{figure}[ht]
    \centering % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{1.png}
  %\caption{image1}
  %\label{fig:1}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{2.png}
  %\caption{image2}
  %\label{fig:2}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{100.png}
  %\caption{image3}
  %\label{fig:3}
\end{subfigure}
%\medskip
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{4000.png}
  %\caption{image4}
  %\label{fig:4}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{9000.png}
  %\caption{image5}
  %\label{fig:5}
\end{subfigure}%\hfil % <-- added
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=\linewidth]{100000.png}
  %\caption{image6}
  %\label{fig:6}
\end{subfigure}
\caption{Forward and backward flows converge to the path with the minimum leakage (shown by blue vertices). Larger dots represent vertices with smaller leakage, and thickness of the green edges corresponds to the flow level. Notice that the paths with smaller leakage get pruned later.}
\label{fig:simulation}
\end{figure}

==> table_non_lin_inc_flow_conv.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{clcc}
\hline
\multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Decision \\ rule\end{tabular}}} &
  \textbf{Graph family} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% instances \\ conv. to a path\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}\% instances \\ conv. to a path \\ with inc. flow\end{tabular}} \\ \hline
\multirow{5}{*}{1.1 power} & $G(n, p)$ local     & 98.7 & 100  \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & Grid                & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{5}{*}{Quadratic} & $G(n, p)$ local     & 96.7 & 100  \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & Grid                & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Quadratic\\ -with-\\ offset\end{tabular}} &
  $G(n, p)$ local &
  98.7 &
  100 \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & Grid                & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{5}{*}{Rank-edge} & $G(n, p)$ local     & 100  & 100  \\
                           & $G(n, p)$ local DAG & 99.3 & 98   \\
                           & Grid                & 94.7 & 72   \\
                           & $G(n, p)$           & 98.7 & 91.3 \\
                           & $G(n, p)$ DAG       & 99.3 & 90.8 \\ \hline
\end{tabular}
\end{table}

==> table_non_lin_leakage_conv.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{clcc}
\hline
\multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Decision \\ rule\end{tabular}}} &
  \textbf{Graph family} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% instances \\ conv. to a path\end{tabular}}} &
  \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}\% instances \\ conv. to a path \\ with leakage\end{tabular}}} \\ \hline
\multirow{4}{*}{1.1 power} & $G(n, p)$ local     & 94   & 100  \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{4}{*}{Quadratic} & $G(n, p)$ local     & 92.7 & 99.3 \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Quadratic\\ -with-\\ offset\end{tabular}} &
  $G(n, p)$ local &
  92 &
  100 \\
                           & $G(n, p)$ local DAG & 100  & 100  \\
                           & $G(n, p)$           & 100  & 100  \\
                           & $G(n, p)$ DAG       & 100  & 100  \\ \hline
\multirow{4}{*}{Rank-edge} & $G(n, p)$ local     & 74   & 31.1 \\
                           & $G(n, p)$ local DAG & 84.1 & 47.9 \\
                           & $G(n, p)$           & 98.7 & 91.3 \\
                           & $G(n, p)$ DAG       & 99.3 & 90.8 \\ \hline
\end{tabular}
\end{table}
